Your Student is Better Than Expected: Adaptive Teacher-Student Collaboration for Text-Conditional Diffusion Models

Knowledge distillation methods have recently shown to be a promising direction to speedup the synthesis of large-scale diffusion models by requiring only a few inference steps. While several powerful distillation methods were recently proposed, the overall quality of student samples is typically lower compared to the teacher ones, which hinders their practical usage. In this work, we investigate the relative quality of samples produced by the teacher text-to-image diffusion model and its distilled student version. As our main empirical finding, we discover that a noticeable portion of student samples exhibit superior fidelity compared to the teacher ones, despite the "approximate" nature of the student. Based on this finding, we propose an adaptive collaboration between student and teacher diffusion models for effective text-to-image synthesis. Specifically, the distilled model produces the initial sample, and then an oracle decides whether it needs further improvements with a slow teacher model. Extensive experiments demonstrate that the designed pipeline surpasses state-of-the-art text-to-image alternatives for various inference budgets in terms of human preference. Furthermore, the proposed approach can be naturally used in popular applications such as text-guided image editing and controllable generation.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Large-scale diffusion probabilistic models (DPMs) have recently shown remarkable success in text-conditional image generation~\cite{podell2023sdxl, rombach2022high, saharia2022photorealistic, nichol2021glide} that aims to produce high quality images closely aligned with the user-specified text prompts.   
However, DPMs pose sequential synthesis leading to high inference costs opposed to feed-forward alternatives, e.g., GANs, that provide  decent text-to-image generation results for a single forward pass~\cite{Sauer2023stylegant, kang2023gigagan}. 

There are two major research directions mitigating the sequential inference problem of state-of-the-art diffusion models. 
One of them considers the inference process as a solution of a probability flow ODE and designs efficient and accurate solvers~\cite{song2020score, karras2022elucidating,lu2022dpm,luu2022dpm, zhao2023unipc} reducing the number of inference steps down to ${\sim}10$ without drastic loss in image quality.
Another direction represents a family of knowledge distillation approaches~\cite{salimans2022progressive, song2023consistency, meng2023distillation, liu2022flow, liu2023instaflow, luo2023latent, gu2023boot} that learn the student model to simulate the teacher distribution requiring only $1{-}4$ inference steps.
Recently, the distillation methods have made a significant step forward~\cite{meng2023distillation, liu2023instaflow, luo2023latent} but still struggle to reach the teacher performance, especially on highly challenging and diverse distributions that are currently standard for text-conditional generation~\cite{schuhmann2022laion}. 
Nevertheless, it is unclear if text-to-image students already have qualitative advantages over their teachers.
If so, perhaps it would be more beneficial to consider a student-teacher collaboration instead of aiming to replace the teacher model entirely. 

In this paper, we take a closer look at images produced by a distilled text-conditional diffusion model and observe that the student can generate some samples even better than the teacher. 
Surprisingly, the number of such samples is significant and sometimes reaches up to half of the empirical distribution.
Based on this observation, we design an adaptive collaborative pipeline that leverages the superiority of student samples and outperforms both individual models alone for various inference budgets.
Specifically, the student model first produces the initial image sample given the text prompt, then the ``oracle'' decides if this sample should be further refined with the teacher model.
%The similar idea has recently demonstrated its effectiveness in the scope of large language models (LLMs)~\cite{frugalgpt} and we show that it can be naturally extended for text-conditional diffusion models as well.
Our approach is schematically presented in \fig{main}.
To summarize, our paper presents the following contributions:

\begin{itemize}
    \item We reveal that the distilled student DPMs can outperform the corresponding teacher DPMs for a noticeable number of generated samples.
    We demonstrate that most of the superior samples correspond to the cases when the student model significantly diverges from the teacher.
    % \item Despite the priority task to approximate the teacher generative process with a few steps, we find that the distilled text-to-image diffusion models can outperform their teachers in a perceptible number of cases.
    % Our analysis reveals that most of these cases occur when the student model largely diverges from the teacher one. 
    %success of the student tends to diverge from the teacher model on the samples which appear more challenging to imitate.  
    %Interestingly, most student successes correspond to these particular cases.
    % Our analysis reveals that the student tends to diverge from the teacher model on the samples which appear more challenging to imitate.  
    % can surpass its teacher in a significant part of cases, although the former learns to mimic the latter using less efforts.
    %Our in-depth analysis reveals that the root of 
    %the superior student performance lies in the divergence from the teacher imitation.
    \item 
    Based on the finding above, we develop an adaptive teacher-student collaborative approach for cost-effective text-to-image synthesis. The method not only increases the inference efficiency but also improves the generative quality by exploiting the superior student samples.
    % We introduce an adaptive teacher-student collaborative approach for cost-effective text-to-image synthesis.
    % The method not only increases the efficiency, but also improves the overall quality by accepting the student samples that are likely to surpass the teacher ones.
    \item We provide an extensive human preference study illustrating the advantages of our approach for text-to-image generation. Moreover, we demonstrate that our pipeline can readily improve the performance of popular text-guided image editing and controllable generation tasks.
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Motivations to consider
% Nevertheless, we assume that not all high-quality samples require the same level of computational effort to be generated.
% Intuitively, the image samples produced for the textual prompts with a small number of typical subjects or the latent variables corresponding to plain scenes may be estimated with fewer computation resources, such as using a distilled model, without perceptual loss in quality.  

% Distilled diffusion models have a trend towards replacing the original models in the applications. 
% Despite the growing popularity, their main drawback is worse performance compared to the fast solvers. 
% Specifically, distillation models cannot achieve the same sample quality as solvers does. 
% The present work looking for approach that allows to combine the distillation speed and solvers quality.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \dmitry{TODO: add a few motivation sentences}

% Large-scale diffusion probabilistic models (DPMs) have recently shown remarkable success in text-conditional image generation that aims to produce high quality images that closely align with the user-specified textual prompts.   
% However, DPMs pose sequential synthesis leading to high inference costs opposed to feed-forward alternatives, e.g., GANs, that provide promising text-to-image generation results for a single forward pass~\cite{stylegant, gigagan}. 

% There are two major directions mitigating the sequential inference problem of state-of-the-art diffusion models. 
% One of them considers the inference process as a solution of a probability flow ODE and designs efficient and accurate solvers~\cite{} that allow reducing the number of inference steps significantly without drastic loss in image quality.
% Also, there is a family of knowledge distillation approaches~\cite{} that learn the student model to simulate the teacher distribution for only $1-4$ inference steps.
% However, these methods still struggle to reach the performance of state-of-the-art diffusion models in terms of image quality or textual alignment.

% Nevertheless, in this paper, we take a closer look at images produced by the distilled models.
% Surprisingly, a significant number of samples have similar or even better quality than the teacher ones. 
% This observation led us to explore the collaborative strategies with the student and teacher models to enhance the overall generative performance having low inference costs.
% In the result, we propose \textit{refining} and \textit{cascading} strategies where the distilled DPM serves as a cheap ``proxy'' model that produces initial samples for a few inference steps.
% The refining approach effectively updates the proxy samples using a few more steps of the original diffusion model.
% The cascading pipeline aims to determine if the initial sample requires regeneration or refinement with a more powerful model.
% We show that this approach can significantly reduce the average inference costs if many initial samples meet the desired quality threshold.
% The overall method combines both strategies together and is presented in \fig{schema}.
% To summarize, our paper provides the following contributions:

% \begin{itemize}
%     \item We explore the samples produced by the state-of-the-art distilled methods and demonstrate that both model produce similar ``simple'' samples but diverge on the more ``complex'' ones. Importantly, some of the student samples appear to be better than the teacher ones and the portion of such samples can be up to $45\%$. 
%     \item We show that the distilled model can serve as a promising initial proxy that surpassing  produced by the distilled model can be refined with the teacher for a few more extra steps.
%     Importantly, the distilled diffusion models benefit from the refinement most compared to other cheap alternatives like GANs, VAEs and efficient solvers. 
%     % This modification can improve the efficiency of the proposed adaptive schema even further.
%     \item We propose the cascading approach using the distilled and original diffusion models and demonstrate the effectiveness of the proposed adaptive sampling strategy on established image benchmarks and text-conditional generation. Notably, the proposed approach leads to both faster inference and higher image fidelity. 
%     \item We reveal that many failure samples produced by the distilled model can be effectively refined with the teacher without expensive regeneration from scratch.
%     This modification can improve the efficiency of the proposed adaptive schema even further.
%     \item We consider various fast alternatives to the distilled models, e.g., GANs and efficient few-step solvers, and observe that the distilled model is the most effective complement to the original model.
% \end{itemize}


==> sec/1_intro_arxiv.tex <==
\section{Introduction}
\label{sec:intro}

Large-scale diffusion probabilistic models (DPMs) have recently shown remarkable success in text-conditional image generation~\cite{podell2023sdxl, rombach2022high, saharia2022photorealistic, nichol2021glide} that aims to produce high quality images closely aligned with the user-specified text prompts.   
However, DPMs pose sequential synthesis leading to high inference costs opposed to feed-forward alternatives, e.g., GANs, that provide  decent text-to-image generation results for a single forward pass~\cite{Sauer2023stylegant, kang2023gigagan}. 

There are two major research directions mitigating the sequential inference problem of state-of-the-art diffusion models. 
One of them considers the inference process as a solution of a probability flow ODE and designs efficient and accurate solvers~\cite{song2020score, karras2022elucidating,lu2022dpm,luu2022dpm, zhao2023unipc} reducing the number of inference steps down to ${\sim}10$ without drastic loss in image quality.
Another direction represents a family of knowledge distillation approaches~\cite{salimans2022progressive, song2023consistency, meng2023distillation, liu2022flow, liu2023instaflow, luo2023latent, gu2023boot, sauer2023adversarial} that learn the student model to simulate the teacher distribution requiring only $1{-}4$ inference steps.
Recently, distilled text-to-image models have made a significant step forward~\cite{meng2023distillation, liu2023instaflow, luo2023latent, sauer2023adversarial}.
However, they still struggle to achieve the teacher performance either in terms of image fidelity and textual alignment~\cite{meng2023distillation, liu2023instaflow, luo2023latent} or distribution diversity~\cite{sauer2023adversarial}.
Nevertheless, we hypothesize that text-to-image students may already have qualitative merits over their teachers.
If so, perhaps it would be more beneficial to consider a teacher-student collaboration rather than focusing on replacing the teacher model entirely.

% \dmitry{reformulate: Recently, the distillation methods have made a significant step forward~\cite{meng2023distillation, liu2023instaflow, luo2023latent, sauer2023adversarial} but still struggle to reach the teacher performance, especially on highly challenging and diverse distributions that are currently standard for text-conditional generation~\cite{schuhmann2022laion}. 
% Nevertheless, it is unclear if text-to-image students already have qualitative advantages over their teachers.
% If so, perhaps it would be more beneficial to consider a student-teacher collaboration instead of aiming to replace the teacher model entirely.}

In this paper, we take a closer look at images produced by distilled text-conditional diffusion models and observe that the student can generate some samples even better than the teacher. 
Surprisingly, the number of such samples is significant and sometimes reaches up to half of the empirical distribution.
Based on this observation, we design an adaptive collaborative pipeline that leverages the superiority of student samples and outperforms both individual models alone for various inference budgets.
Specifically, the student model first generates an initial image sample given a text prompt, and then an ``oracle'' decides if this sample should be updated using the teacher model at extra compute.
The similar idea has recently demonstrated its effectiveness for large language models (LLMs)~\cite{chen2023frugalgpt} and we show that it can be naturally applied to text-conditional diffusion models as well.
Our approach is schematically presented in \fig{main}.
To summarize, our paper presents the following contributions:
%aims to determine if this sample is likely to be better than the teacher one generated for the same text prompt and initial noise.

\begin{itemize}
    \item We reveal that the distilled student DPMs can outperform the corresponding teacher DPMs for a noticeable number of generated samples.
    We demonstrate that most of the superior samples correspond to the cases when the student model significantly diverges from the teacher.
    \item 
    Based on the finding above, we develop an adaptive teacher-student collaborative approach for effective text-to-image synthesis. The method not only reduces the average inference costs but also improves the generative quality by exploiting the superior student samples.
    \item We provide an extensive human preference study illustrating the advantages of our approach for text-to-image generation. Moreover, we demonstrate that our pipeline can readily improve the performance of popular text-guided image editing and controllable generation tasks.
\end{itemize}

==> sec/2_related.tex <==
\section{Related work}

\textbf{Diffusion Probabilistic Models} (DPMs)~\cite{ho2020denoising, song2019generative, song2020score} represent a class of generative models consisting of \textit{forward} and  \textit{reverse} processes.
The \textit{forward} process $\{\boldsymbol{x}_t\}_{[0, T]}$ transforms real data $\boldsymbol{x}_{0} \sim p_{\text{data}}(\boldsymbol{x}_{0})$ into the noisy samples $\boldsymbol{x}_{t}$ using the transition kernels
$\mathcal{N}\left(\boldsymbol{x}_{t} \ | \ \sqrt{1 - \sigma^2_{t}} \boldsymbol{x}_{0}, \sigma^2_{t} \mathbf{I} \right)
    \label{eq:forward_transition}$
specifying $\sigma_t$ according to the selected \textit{noise schedule}.
%There are two prevalent special cases of diffusion processes: \textit{variance-preserving} (VP) and \textit{variance-exploding} (VE)\cite{scoresde}, where $\alpha_t = \sqrt{1 - \sigma^2_t}$ and $\alpha^2_t = 1$, respectively.
%The popular open-source text-conditional models, e.g., Stable Diffusion~\cite{}, usually operate with VP processes. 

The \textit{reverse} diffusion process generates new data points by gradually denoising samples from a simple (usually standard normal) distribution.
This process can be formulated as a \textit{probabilistic-flow ODE} (PF-ODE)~\cite{song2020denoising, song2020score}, where 
the only unknown component is a \textit{score function}, which is approximated with a neural network.
The ODE perspective of the reverse process fosters designing a wide range of the specialized solvers~\cite{lu2022dpm, zhao2023unipc, luu2022dpm, song2020denoising, karras2022elucidating, zhang2022fast, jolicoeur2021gotta} for efficient and accurate sampling.
However, for text-to-image generation, one still needs ${\sim}25$ and more steps for the top performance. 
% \begin{equation}
%     \begin{gathered}
%         \mathrm{d}\boldsymbol{x}= \left[\boldsymbol{f}(t)\boldsymbol{x}_t - g^2(t) \nabla_{\boldsymbol{x}}\log p_{t}(\boldsymbol{x}_t)\right]\mathrm{d}t,
%     \end{gathered} 
%     \label{eq:reverse_ode}
% \end{equation}
% where $f(t){=}\frac{\mathrm{d}\log \alpha_t}{\mathrm{d}t}$ and $g^2(t){=} \frac{\mathrm{d} \sigma^2_t}{\mathrm{d}t} - 2 \frac{\mathrm{d}\log \alpha_t}{\mathrm{d}t}\sigma^2_t$~\cite{vdp}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TODO: move it to analysis/experiments (setup description)
% In our work, we use DDIM~\cite{} and DPM-Solver~\cite{dpm2} as sampling methods. 
% DPM-Solver is described in detail in \ref{app:fast_solvers}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Text-conditional diffusion models} %inject the textual information into a neural network via textual embedding extracted using a text-encoder, e.g., CLIP~\cite{radford2021learning}. 
%To attain a trade-off between sample quality and diversity, the classifier-free~\cite{ho2022classifier} or classifier guidance~\cite{dhariwal2021diffusion} can be applied. 
can be largely grouped into \textit{cascaded} and \textit{latent} diffusion models. 
The cascaded models~\cite{saharia2022photorealistic, nichol2021glide} generate a sample in several stages using separate diffusion models for different image resolutions.
The latent diffusion models~\cite{podell2023sdxl, rombach2022high, ramesh2021zero} first generate a low-resolution latent variable in the VQVAE~\cite{van2017neural} space and then apply its feedforward decoder to map the latent sample to the high-resolution pixel space. 
Thus, the latent diffusion models have significantly more efficient inference thanks to a single forward pass for the upscaling step.  

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\linewidth]{images/student_better_teacher.jpg}
    \captionof{figure}{\textbf{Student outperforms its teacher}. \textit{Left:}  Text-conditional image synthesis. \textit{Right:} Text-guided image editing (SDEdit~\cite{meng2021sdedit}). The images within each pair are generated for the same initial noise sample.} 
    \label{fig:student_better_teacher}
\end{figure*}

Along with cascaded models, there are other works combining several diffusion models into a single pipeline.
Some methods propose using distinct diffusion models at different time steps~\cite{balaji2022ediffi, liu2023oms, feng2023ernie, xue2023raphael}.
Others ~\cite{podell2023sdxl, liu2023instaflow} consider an additional model to refine the samples produced with a main model. 
In contrast, our method relies on the connection between student and teacher models and adaptively improves only selected student samples to reduce the inference costs.

Text-to-image diffusion models have also succeeded in text-guided image editing and personalization~\cite{brooks2023instructpix2pix, meng2021sdedit, mokady2022null, kawar2023imagic, ruiz2022dreambooth, gal2022textual}. 
Moreover, some methods allow controllable generation via conditioning on additional inputs, e.g., canny-edges, semantic masks, sketches~\cite{zhang2023adding, voynov2023sketch}.
Our experiments show that the proposed pipeline is well-suited to these techniques. 

\textbf{Distillation of diffusion models} is another pivotal direction for efficient diffusion inference~\cite{song2023consistency, song2023improved, salimans2022progressive, meng2023distillation, berthelot2023tract, liu2023instaflow}. 
The primary goal is to adapt the diffusion model parameters to produce teacher quality samples for $1{-}4$ steps. 
Recently, consistency distillation (CD)~\cite{song2023consistency} have demonstrated promising results on both classical benchmarks~\cite{kim2023consistency} and text-to-image generation~\cite{luo2023latent}.
Nevertheless, the distilled models still fall short of the teacher performance for image generation~\cite{song2023consistency}.
Therefore,  it is not entirely clear if a few-step student can perfectly approximate the teacher without loss in image fidelity, diversity or textual alignment in the future. 
%The present work suggests considering the distilled models in another role: 
%not as a few-step teacher alternative but as a strong companion in the top-performing collaboration.
% for  focuses on the approach that combines the strengths of the student and teacher models into the unified generative pipeline.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TODO: move it to analysis/experiments (setup description)
% Therefore, in our work, we train the latent consistency model~\cite{lcm} for StableDiffusion v1.5 on the filtered 80M subset of the LAION2B dataset~\cite{}. 
% The detailed CD overview, our distillation pipeline and hyperparameters are thoroughly described in \app{cd_training}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% TODO: describe the distill methods that reduce the model size.


%Diffusion Models (DMs) are a class of generative models gradually producing samples from a simple (usually standard normal) distribution. 
%Despite the great quality of produced samples, the generation procedure is bottlenecked by iterative neural network utilization. 
% The overall framework of diffusion models can be separated into three parts: \textit{forward}, \textit{backward} processes and \textit{score approximation}.
% , and obeys the following equation:
% \begin{equation}
%     \begin{gathered}
%         \mathrm{d}\boldsymbol{x}= \boldsymbol{f}(\boldsymbol{x}, t)\mathrm{d}t + g(t)\mathrm{d}\boldsymbol{w}_{t}, t \in [0, T].
%     \end{gathered}\label{background:forward_sde}
% \end{equation}
% Here $\boldsymbol{f}(\boldsymbol{x}, t)$, $g(t)$ are the drift and diffusion coefficient, respectively, and $\mathrm{d}\boldsymbol{w}_{t}$ is the infinitesimal Brownian motion. 
% One of the common choices is $\boldsymbol{f}(\boldsymbol{x}, t) = 0, \ g(t) = \sqrt{\frac{\mathrm{d}\sigma^2_{t}}{\mathrm{d}t}}$. 
% Thus, the forward equation has a closed-form solution, which transforms the real data with the respect to the transition kernels $ p_{t}\left(\boldsymbol{x}_{t} \ | \  \boldsymbol{x}_{0}\right) = \mathcal{N}\left(\boldsymbol{x}_{t} \ | \boldsymbol{x}_{0}, \sigma^2_{t}\mathbf{I} \right).$

% To generate the data, the \textit{reverse} diffusion process was formulated.
% \begin{equation}
%     \begin{gathered}
%         \mathrm{d}\boldsymbol{x}= \left[\boldsymbol{f}(\boldsymbol{x}, t) - g(t)^{2} \nabla_{\boldsymbol{x}}\log p_{t}(\boldsymbol{x})\right]\mathrm{d}t
%     \end{gathered} \label{background:reverse_ode}
% \end{equation}
% The complexity is dictated by unknown function $\log p_{t}(\boldsymbol{x})$ typically called as the score function. Since its explicit form is unable to calculate, \textit{score approximation} is utilized where a neural network $\boldsymbol{x}_{\theta}(\boldsymbol{x}, t)$ learns to predict the conditional expectation $\mathbb{E} \left[\boldsymbol{x}_{0}|\boldsymbol{x}\right]$.

% The unsolvability of the equation (\ref{background:reverse_ode}) for complex data causes the need to use numerical integrators. However, there is a well-establish ODE-solvers framework, which is widely used in the literature. The paper mainly builds upon the recent high-end solvers, EDM and DPM-solver, which described in detail in \ref{app:fast_solvers}. Despite the increased attention to the fast solvers, diffusion models are still unable to generate good samples in the low-step regime (1-10 NFE). \\ 

==> sec/2_related_arxiv.tex <==
\section{Related work}

\textbf{Diffusion Probabilistic Models} (DPMs)~\cite{ho2020denoising, song2019generative, song2020score} represent a class of generative models consisting of \textit{forward} and  \textit{reverse} processes.
The \textit{forward} process $\{\boldsymbol{x}_t\}_{[0, T]}$ transforms real data $\boldsymbol{x}_{0} \sim p_{\text{data}}(\boldsymbol{x}_{0})$ into the noisy samples $\boldsymbol{x}_{t}$ using the transition kernels
$\mathcal{N}\left(\boldsymbol{x}_{t} \ | \ \sqrt{1 - \sigma_{t}} \boldsymbol{x}_{0}, \sigma_{t} \mathbf{I} \right)
    \label{eq:forward_transition}$
specifying $\sigma_t$ according to the selected \textit{noise schedule}.
%There are two prevalent special cases of diffusion processes: \textit{variance-preserving} (VP) and \textit{variance-exploding} (VE)\cite{scoresde}, where $\alpha_t = \sqrt{1 - \sigma^2_t}$ and $\alpha^2_t = 1$, respectively.
%The popular open-source text-conditional models, e.g., Stable Diffusion~\cite{}, usually operate with VP processes. 

The \textit{reverse} diffusion process generates new data points by gradually denoising samples from a simple (usually standard normal) distribution.
This process can be formulated as a \textit{probabilistic-flow ODE} (PF-ODE)~\cite{song2020denoising, song2020score}, where 
the only unknown component is a \textit{score function}, which is approximated with a neural network.
The ODE perspective of the reverse process fosters designing a wide range of the specialized solvers~\cite{lu2022dpm, zhao2023unipc, luu2022dpm, song2020denoising, karras2022elucidating, zhang2022fast, jolicoeur2021gotta} for efficient and accurate sampling.
However, for text-to-image generation, one still needs ${\sim}25$ and more steps for the top performance. 
% \begin{equation}
%     \begin{gathered}
%         \mathrm{d}\boldsymbol{x}= \left[\boldsymbol{f}(t)\boldsymbol{x}_t - g^2(t) \nabla_{\boldsymbol{x}}\log p_{t}(\boldsymbol{x}_t)\right]\mathrm{d}t,
%     \end{gathered} 
%     \label{eq:reverse_ode}
% \end{equation}
% where $f(t){=}\frac{\mathrm{d}\log \alpha_t}{\mathrm{d}t}$ and $g^2(t){=} \frac{\mathrm{d} \sigma^2_t}{\mathrm{d}t} - 2 \frac{\mathrm{d}\log \alpha_t}{\mathrm{d}t}\sigma^2_t$~\cite{vdp}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TODO: move it to analysis/experiments (setup description)
% In our work, we use DDIM~\cite{} and DPM-Solver~\cite{dpm2} as sampling methods. 
% DPM-Solver is described in detail in \ref{app:fast_solvers}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Text-conditional diffusion models} %inject the textual information into a neural network via textual embedding extracted using a text-encoder, e.g., CLIP~\cite{radford2021learning}. 
%To attain a trade-off between sample quality and diversity, the classifier-free~\cite{ho2022classifier} or classifier guidance~\cite{dhariwal2021diffusion} can be applied. 
can be largely grouped into \textit{cascaded} and \textit{latent} diffusion models. 
The cascaded models~\cite{saharia2022photorealistic, nichol2021glide} generate a sample in several stages using separate diffusion models for different image resolutions.
The latent diffusion models~\cite{podell2023sdxl, rombach2022high, ramesh2021zero} first generate a low-resolution latent variable in the VAE~\cite{kingma2013auto} space and then apply its feedforward decoder to map the latent sample to the high-resolution pixel space. 
Thus, the latent diffusion models have significantly more efficient inference thanks to a single forward pass for the upscaling step.  

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\linewidth]{images/student_better_teacher.jpg}
    \vspace{-6mm}
    \captionof{figure}{\textbf{Student outperforms its teacher (SD1.5)}. \textit{Left:}  Text-conditional image synthesis. \textit{Right:} Text-guided image editing (SDEdit~\cite{meng2021sdedit}). The images within each pair are generated for the same initial noise sample.} 
    \label{fig:student_better_teacher}
\end{figure*}

Along with cascaded models, there are other works combining several diffusion models into a single pipeline.
Some methods propose to use distinct diffusion models at different time steps~\cite{balaji2022ediffi, liu2023oms, feng2023ernie, xue2023raphael}.
Others~\cite{podell2023sdxl, liu2023instaflow} consider an additional model to refine the samples produced with a base model. 
In contrast, our method relies on the connection between student and teacher models and adaptively improves only selected student samples to reduce the inference costs.

Text-to-image diffusion models have also succeeded in text-guided image editing and personalization~\cite{brooks2023instructpix2pix, meng2021sdedit, mokady2022null, kawar2023imagic, ruiz2022dreambooth, gal2022textual}. 
Moreover, some methods allow controllable generation via conditioning on additional inputs, e.g., canny-edges, semantic masks, sketches~\cite{zhang2023adding, voynov2023sketch}.
Our experiments show that the proposed pipeline is well-suited to these techniques. 

\textbf{Distillation of diffusion models} is another pivotal direction for efficient diffusion inference~\cite{song2023consistency, song2023improved, salimans2022progressive, meng2023distillation, berthelot2023tract, liu2023instaflow, sauer2023adversarial}. 
The primary goal is to adapt the diffusion model parameters to represent the teacher image distribution for $1{-}4$ steps. 
Recently, consistency distillation (CD)~\cite{song2023consistency} have demonstrated promising results on both classical benchmarks~\cite{kim2023consistency, song2023improved} and text-to-image generation~\cite{luo2023latent} but fall short of the teacher performance at the moment.
Concurrently, adversarial diffusion distillation~\cite{sauer2023adversarial} 
could outperform the SDXL-Base~\cite{podell2023sdxl} teacher for $4$  steps in terms of image quality and prompt alignment.
However, it significantly reduces the diversity of generated samples, likely due to the adversarial training~\cite{goodfellow2020generative} and mode-seeking distillation technique~\cite{poole2023dreamfusion}.
Therefore, it is still an open question if a few-step distilled model can perfectly approximate the diffusion model on highly challenging and diverse distributions that are currently standard for text-conditional generation~\cite{schuhmann2022laion}.  

% Nevertheless, the distilled models still fall short of the teacher performance for image generation~\cite{song2023consistency}.

==> sec/3_method.tex <==
\section{Toward a unified teacher-student framework} \label{main_analysis}

Opposed to the ultimate purpose of replacing the expensive text-to-image diffusion models with more effective few-step alternatives, the present work suggests considering the distilled text-to-image models as a firm companion in teacher-student collaboration.

In this section, we first explore the advantages of the distilled text-to-image models and then unleash their potential in a highly effective generative pipeline comprising the student and teacher models. 

\subsection{Delving deeper into the student performance} 
We start with a side-by-side comparison of the student and teacher text-to-image diffusion models. 
Here, we focus on Stable Diffusion v1.5\footnote{https://huggingface.co/runwayml/stable-diffusion-v1-5} as our main teacher model and distill it using consistency distillation~\cite{song2023consistency}.
The student details and sampling setup are presented in~\ref{app:analysis}.
We also investigate the recent latent consistency model~\cite{luo2023latent} distilled from Dreamshaper v7\footnote{https://huggingface.co/Lykon/dreamshaper-7} in~\ref{app:analysis}.
\begin{figure}[ht!]
    \centering
\includegraphics[width=1.0\linewidth]{images/dual_model_beh.jpg}
    \vspace{-2mm}
    \caption{(a) Visual examples of similar (Left) and dissimilar (Right) teacher and student samples. 
    (b) Similarity between student and teacher samples w.r.t. the difference in sample quality. Highly distinct samples tend to be of different quality. 
    (c) Human vote distributions for different distance ranges between student and teacher samples. Most student wins are achieved when the student diverges from the teacher.}
    \label{fig:dual_mode_beh}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/complexity_distance_diverse.jpg}
    \vspace{-6mm}
    \caption{\textbf{Effect of image complexity}. 
    (a) More similar student and teacher samples corresponds to simpler images and vice versa. 
    (b) The student and teacher largely diverge in image quality on the complex teacher samples. Notably, the student often outperforms the teacher on these samples.}
    \label{fig:image_complexity}
\end{figure} 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/prompts_analysis.jpg}
    \vspace{-6mm}
    \caption{\textbf{Effect of text prompts}. 
    (a) Shorter prompts usually lead to more similar student and teacher samples.
    (b) The student and teacher tend to generate more similar images when the student relies heavily on the text prompt.}
    \label{fig:prompts}
\end{figure} 

%\begin{figure*}[t!]
%    \centering
%    \includegraphics[width=\linewidth]{images/image_synth_ours_teacher.jpg}
%    \captionof{figure}{Visual examples produced with our adaptive approach and the teacher model (DDIM50). } 
%    \label{fig:ours_teacher_generation}
%\end{figure*}

In \fig{main}~(Right), we provide the human votes for 600 random text prompts from COCO2014~\cite{lin2014microsoft} and DiffusionDB~\cite{wangDiffusionDBLargescalePrompt2022} for StableDiffusion and Dreamshaper, respectively.
The images within each pair are generated for the same initial noise sample.
We observe that the students generally falls short of the teacher performance.
However, interestingly, despite the initial intention to mimic the teacher model, ${\sim}30\%$ student samples were preferred over the teacher ones.
A few visual examples in ~\fig{student_better_teacher} validate these results.
% More examples are in \ref{app:analysis}. 
Therefore, we can formulate our first observation:
\begin{tcolorbox}[colback=red!5!white,colframe=black!75!black]
The student can surpass its teacher on a substantial portion of image samples.\end{tcolorbox} 
Below, we develop a more profound insight into this phenomenon.
% For evaluation, we consider 5000 prompts from the COCO2014~\cite{} validation split and a random subset of 600 prompts for human evaluation.
% Note that we align the student and teacher samples by fixing the initial noise sample $x_T\sim N(0,I)$ within each prompt.
% Concurrently, \citet{lcm} have realised the latent consistency model distilled from DreamShaper v7~\cite{}.
% We provide the similar analysis for this model in \app{dreamshaper}.
% There is also publicly available single-step InstaFlow~\cite{} model but it fails to produce satisfactory samples in our experiments.
\\ \textbf{Student-teacher similarity.}
First, we evaluate the student's ability to imitate the teacher.
We compute pairwise similarities between the student and teacher images generated for the same text prompts and initial noise.
As a similarity measure, we consider DreamSim~\cite{fu2023dreamsim} tuned to align with human perception judgments. 
For evaluation, we consider 5000 prompts from the COCO2014~\cite{lin2014microsoft} validation split.

Primarily, we observe that many student samples are highly distinct from the teacher ones. 
A few image pairs are presented in Figure~\ref{fig:dual_mode_beh}a. 
\fig{dual_mode_beh}c presents the human vote distribution over three distance ranges: low, medium, and high.
Interestingly, most student wins appear when its samples are highly different from the teacher ones. 
This brings us to our second observation:
\begin{tcolorbox}[colback=red!5!white,colframe=black!75!black]
The student wins are more likely where its samples significantly differ from the teacher ones.  \end{tcolorbox}

Also, we evaluate the relative gap in sample quality against the similarity between the teacher and student outputs.
To measure the quality of individual samples, we use ImageReward~\cite{xu2023imagereward}, which shows a positive correlation with human preferences in terms of image fidelity and textual alignment. 
The gap in sample quality is calculated as the difference between ImageReward scores for student and teacher samples.
We observe that highly distinct samples likely have a significant difference in image quality.
Importantly, this holds for both student failures and successes, as shown in \fig{dual_mode_beh}b.
Therefore, by effectively detecting the positive student samples and improving the negative ones, we can potentially increase the overall generative performance. 
\\ \textbf{Image complexity.}
Then, we describe the connection of the similarity between student and teacher samples with the teacher image complexity. 
To estimate the latter, we use the recent ICNet model~\cite{feng2023ic9600} learned on a large-scale human annotated dataset.  
The results are presented in \fig{image_complexity}. 
We notice that larger distances between student and teacher outputs are more typical for complex teacher samples. 
In other words, the student mimics its teacher for plain images, e.g., close-up faces, while acting more as an independent model for more intricate ones. 
In addition, \fig{image_complexity}b confirms that significant changes in image quality are observed for more complex images.
\\ \textbf{Text prompts.}
Then, we analyse the connection of the student-teacher similarity with the prompt length.
\fig{prompts} demonstrates that shorter prompts typically lead to more similar teacher and student samples.
The prompt length equals to the number of CLIP tokens. 
Intuitively, longer prompts are more likely to describe intricate scenes and object compositions than shorter ones.
Note that long prompts may carry various textual informativeness and describe concepts of different complexity.  
We hypothesize that this causes high variance in student-teacher similarity. 

Also, we report the prompt influence on the student generation w.r.t. the student-teacher similarity in \fig{prompts}b. 
We estimate the prompt influence by aggregating student cross-attention maps. 
More details are in \ref{app:analysis}.
The student tends to imitate the teacher if it relies heavily on the text prompt.
\\ \textbf{Trajectory curvature.}
Previously, it was shown to be beneficial to straighten the PF-ODE trajectory before distillation~\cite{liu2022flow,liu2023instaflow}. 
We investigate the effect of the trajectory curvature on the similarity between the teacher and student samples and its correlation with the teacher sample complexity. 
We calculate the trajectory curvatures following ~\cite{chen2023geometric} and observe that straighter trajectories lead to more similar student and teacher samples (\fig{curvature},a). 
In addition, we show, for the first time, that the trajectory curvature correlates with the teacher sample complexity (\fig{curvature},b).
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/curvature.jpg}
    \vspace{-6mm}
    \caption{\textbf{Effect of teacher trajectory curvature}. 
    (a) The student samples resemble the teacher ones for less curved trajectories. 
    (b) Straighter trajectories usually correspond to plainer teacher images.}
    \label{fig:curvature}
\end{figure} 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/no-ref.jpg}
    \caption{\textbf{Full-reference vs no-reference decision-making}. Usually, one can find a $k$-th percentile of the ImageReward scores providing the correlation with human votes similar to the full-reference comparisons but without observing the teacher samples}
    %Usually, there is a percentile providing the same correlation as the full-reference estimate without seeing a teacher sample.}
    \label{fig:ref_no_ref}
\end{figure} 

To sum up, we conclude that the student largely diverges from the teacher on the samples that are challenging in different respects.
Interestingly, the student can regularly outperform the teacher in these cases.

% This behavior resembles deep ensembles~\cite{} where a bunch of independently trained models provide diverse predictions on the complex inputs and increase the overall performance.
% However, in our case, the distilled model initialized with the teacher weights and learnt to imitate the teacher still can produce sufficient diverse samples to significantly improve the teacher performance.
% We hypothesize that it is caused by the highly stochastic nature of the diffusion models and consistency distillation methods.


\subsection{Method}

In this section, we propose an adaptive collaborative approach consisting of three steps:
1) Generate a sample with the student;
2) Adaptively decide if the sample needs further improvement or not;
3) If so, improve the sample with the teacher model.

\textbf{Student generation step} produces an initial sample $\mathcal{X}^{\mathbf{S}}$ for a given context and noise.
In our work, we consider consistency distillation as a student model and use the multistep consistency sampling algorithm~\cite{song2023consistency} for generation.

\textbf{Adaptive step} leverages our finding that many student samples may exhibit superior quality.
Specifically, we seek an ``oracle'' that correctly detects superior student samples. 
We use an individual sample quality estimator $\mathbf{E}$ that returns scores correlating with human votes. 
In our work, we consider the current state-of-the-art automated estimator, ImageReward (IR)~\cite{xu2023imagereward} that is learned to imitate the text-to-image human preference.

Then, comparing the scores of the teacher and student samples, one can decide which one is better.
However, in practice, we avoid expensive teacher inference to preserve the efficiency of our approach.
Therefore, a decision must be made having access only to the initial student sample $\mathcal{X}^{\mathbf{S}}$. 
To address this problem, we introduce a cut-off threshold $\tau$  tuned on a hold-out subset as a $k$-th percentile of the IR scores. 
Interestingly, we observe that it is possible to reproduce the accuracy of the full-reference estimation by varying $\tau$ (see \fig{ref_no_ref}). 

During inference, the IR score is calculated only for $\mathcal{X}^{\mathbf{S}}$.
If it exceeds the threshold $\tau$, we accept the sample and avoid further teacher involvement. 
Note that IR calculation costs are negligible compared to a single diffusion step, see \ref{app:method}.

\textbf{Improvement step} engages the teacher to improve the quality of the rejected student samples.
We consider two teacher involvement strategies: \textit{regeneration} and \textit{refinement}. 
The former simply applies the teacher model to produce a novel sample from scratch for the same text prompt and noise.
The refinement is inspired by the recent work~\cite{podell2023sdxl}. 
Specifically, $\mathcal{X}^{\mathbf{S}}$ is first corrupted with a Gaussian noise controlled by the rollback value $\sigma \in [0, 1]$. 
Higher $\sigma$ leads to more pronounced changes. 
We vary $\sigma$ between $0.4$ and $0.75$ in our experiments.
Then, the teacher starts sampling from the corrupted sample following the original noise schedule and using an arbitrary solver, e.g., DPM-Solver~\cite{lu2022dpm}.
Note that refinement requires significantly fewer steps to produce the final sample than generation from scratch. Intuitively, the refinement strategy aims to fix the defects in the student sample.
At the same time, the regeneration strategy may be useful if $\mathcal{X}^{\mathbf{S}}$ is poorly aligned with the text prompt in general.
Our experiments confirm this intuition. %that refinement generally enhances image fidelity while regeneration leads to better textual alignment. 

%According to our observations in ~\fig{}b, if the student already generates a high quality sample, it is likely that the teacher will not beat this sample and hence we do not need to spend extra compute for the teacher inference.
% Therefore, one needs an ``oracle'' that makes a decision if the student sample is better than the teacher one. 
%already poses high fidelity and textual alignment.% or leave it to the teacher. 

%\begin{algorithm}[t!]
%\DontPrintSemicolon
%  
%  \KwInput{$\mathbf{E}, \mathbf{S}, \mathbf{T} - $ estimator, student, teacher; \\ $\mathcal{I} - $ input; $\sigma, \tau - $ rollback value and cut-off threshold.}
%  \vspace{1.5mm}
%  $\hat{\mathcal{O}} = \mathbf{S}(\mathcal{I})$ \tcp*{Student prediction}
%  \vspace{1.5mm}
%  \If{$\mathbf{E}(\hat{\mathcal{O}}) < \tau$}
%  {
%    \vspace{1.5mm}
%    \textit{Strategy 1}: \tcp*{Refinement}
%       \ \ \ \ $\hat{\mathcal{O}}_{\sigma} = (1 - \sigma) \cdot \hat{\mathcal{O}} + \sigma \cdot Z$ \tcp*{Noising}
%       \ \ \ \ $\hat{\mathcal{O}} = \mathbf{T}(\mathcal{I}, \hat{\mathcal{O}}_{\sigma})$ \\
%    \textit{Strategy 2}: \tcp*{Generation using teacher}
%        \ \ \ \ $\hat{\mathcal{O}} = \mathbf{T}%(\mathcal{I})$ 
%  } 
%  {\Return{$\hat{\mathcal{O}}$}}
%\caption{teacher-student adaptive collaboration}
%\label{alg:method_alg}
%\end{algorithm}

%We present the overall adaptive collaborative pipeline in \alg{method_alg}.

% One potential limitation of the proposed approach is poor correlation of existing automated text-to-image estimators with human preference.
% For example, IR exhibits up to $65 \%$ correlation with the annotators. 
% In Section~\ref{subsec:image_synth}, we investigate how the accuracy of the automated estimator affects the performance of our scheme and demonstrate the potential of the proposed method if more accurate estimators are developed in the future work. 


==> sec/3_method_arxiv.tex <==
\section{Toward a unified teacher-student framework} \label{main_analysis}

Opposed to the purpose of replacing the expensive text-to-image diffusion models by more effective few-step alternatives, the present work suggests considering the distilled text-to-image models as a firm companion in a teacher-student collaboration.

In this section, we first explore the advantages of the distilled text-to-image models and then unleash their potential in a highly effective generative pipeline comprising the student and teacher models. 

\subsection{Delving deeper into the student performance} 
We start with a side-by-side comparison of the student and teacher text-to-image diffusion models. 
Here, we focus on Stable Diffusion v1.5\footnote{https://huggingface.co/runwayml/stable-diffusion-v1-5} (SD$1.5$) as our main teacher model and distill it using consistency distillation~\cite{song2023consistency}.
The student details and sampling setup are presented in~\ref{app:student_details}.
The similar analysis for a few other distilled models is provided in~\ref{app:other_distill}.
% We also investigate the recent latent consistency model~\cite{luo2023latent} distilled from Dreamshaper v7\footnote{https://huggingface.co/Lykon/dreamshaper-7} in~\ref{app:analysis}.

\begin{figure}[ht!]
    \centering
    \vspace{-1mm}
\includegraphics[width=1.0\linewidth]{images/dual_model_beh.jpg}
    \vspace{-7mm}
    \caption{(a) Visual examples of similar (Left) and dissimilar (Right) teacher and student samples. 
    (b) Similarity between the student and teacher samples w.r.t. the difference in sample quality. 
    Highly distinct samples tend to be of different quality. 
    (c) Human vote distribution for different distance ranges between student and teacher samples. Most of the student wins are achieved when the student diverges from the teacher.
    %(*) The histograms represent individual distributions and are not comparable between each other.
    }
    \vspace{-1mm}
    \label{fig:dual_mode_beh}
\end{figure}
\begin{figure}[t!]
    \centering
    \vspace{2mm}
    \includegraphics[width=1.0\linewidth]{images/complexity_distance_diverse.jpg}
    \vspace{-6mm}
    \caption{\textbf{Effect of image complexity}. 
    (a) More similar student and teacher samples corresponds to simpler images and vice versa. 
    (b) The student and teacher largely diverge in image quality on the complex teacher samples. }
    \label{fig:image_complexity}
\end{figure} 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/prompts_analysis.jpg}
    \vspace{-6mm}
    \caption{\textbf{Effect of text prompts}. 
    (a) Shorter prompts usually lead to more similar student and teacher samples.
    (b) The student and teacher tend to generate more similar images when the student relies heavily on the text prompt.}
    \label{fig:prompts}
\end{figure}

In \fig{main}~(Right), we provide the human votes for 600 random text prompts from COCO2014~\cite{lin2014microsoft} for SD$1.5$  and SDXL.
The images within each pair are generated for the same initial noise sample.
We observe that the students generally falls short of the teacher performance.
However, interestingly, despite the initial intention to mimic the teacher model, ${\sim}30\%$ student samples were preferred over the teacher ones.
A few visual examples in ~\fig{student_better_teacher} validate these results.
% More examples are in \ref{app:analysis}. 
Therefore, we can formulate our first observation:
\begin{tcolorbox}[colback=red!5!white,colframe=black!75!black]
The student can surpass its teacher in a substantial portion of image samples.\end{tcolorbox} 
Below, we develop a more profound insight into this phenomenon.
% For evaluation, we consider 5000 prompts from the COCO2014~\cite{} validation split and a random subset of 600 prompts for human evaluation.
% Note that we align the student and teacher samples by fixing the initial noise sample $x_T\sim N(0,I)$ within each prompt.
% Concurrently, \citet{lcm} have realised the latent consistency model distilled from DreamShaper v7~\cite{}.
% We provide the similar analysis for this model in \app{dreamshaper}.
% There is also publicly available single-step InstaFlow~\cite{} model but it fails to produce satisfactory samples in our experiments.
\\ \textbf{Student-teacher similarity.}
First, we evaluate the student's ability to imitate the teacher.
We compute pairwise similarities between the student and teacher images generated for the same text prompts and initial noise.
As a similarity measure, we consider DreamSim~\cite{fu2023dreamsim} tuned to align with the human perception judgments. 
For evaluation, we consider 5000 prompts from the COCO2014~\cite{lin2014microsoft} validation split.

Primarily, we observe that many student samples are highly distinct from the teacher ones. 
A few image pairs are presented in Figure~\ref{fig:dual_mode_beh}a. 
\fig{dual_mode_beh}c presents the human vote distribution for three distance ranges: low, medium, and high.
Interestingly, most of the student wins appear when its samples are highly different from the teacher ones. 
This brings us to our second observation:
\begin{tcolorbox}[colback=red!5!white,colframe=black!75!black]
The student wins are more likely where its samples significantly differ from the teacher ones.  \end{tcolorbox}

Also, we evaluate the relative gap in sample quality against the similarity between the teacher and student outputs.
To measure the quality of individual samples, we use ImageReward~\cite{xu2023imagereward}, which shows a positive correlation with human preferences in terms of image fidelity and prompt alignment. 
The gap in sample quality is calculated as the difference between the ImageReward scores for student and teacher samples.
We observe that highly distinct samples likely have a significant difference in quality.
Importantly, this holds for both student failures and successes, as shown in \fig{dual_mode_beh}b.
Therefore, effectively detecting the positive student samples and improving the negative ones can potentially increase the generative performance. 
\\ \textbf{Image complexity.}
Then, we describe the connection of the similarity between student and teacher samples with the teacher image complexity. 
To estimate the latter, we use the ICNet model~\cite{feng2023ic9600} learned on a large-scale human annotated dataset.  
The results are presented in \fig{image_complexity}. 
We notice that larger distances between student and teacher outputs are more typical for complex teacher samples. 
In other words, the student mimics its teacher for plain images, e.g., close-up faces, while acting more as an independent model for more intricate ones. 
\fig{image_complexity}b confirms that significant changes in image quality are observed for more complex images.
\\ \textbf{Text prompts.}
Then, we analyse the connection of the student-teacher similarity with the prompt length.
\fig{prompts} demonstrates that shorter prompts typically lead to more similar teacher and student samples.
Here, the prompt length equals to the number of CLIP tokens. 
Intuitively, longer prompts are more likely to describe intricate scenes and object compositions than shorter ones.
Note that long prompts can also carry low textual informativeness and describe concepts of low complexity. 
We hypothesize that this causes high variance in \fig{prompts}a. 

Also, we report the prompt influence on the student generation w.r.t. the student-teacher similarity in \fig{prompts}b. 
We estimate the prompt influence by aggregating student cross-attention maps. 
More details are in \ref{app:calc_details}.
The student tends to imitate the teacher if it relies heavily on the text prompt.
\\ \textbf{Trajectory curvature.}
Previously, it was shown to be beneficial to straighten the PF-ODE trajectory before distillation~\cite{liu2022flow,liu2023instaflow}. 
We investigate the effect of the trajectory curvature on the similarity between the teacher and student samples and its correlation with the teacher sample complexity. 
We estimate the trajectory curvatures following~\cite{chen2023geometric} and observe that straighter trajectories lead to more similar student and teacher samples (\fig{curvature}a). 
In addition, we show that the trajectory curvature correlates with the teacher sample complexity (\fig{curvature}b).

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/curvature.jpg}
    \vspace{-6mm}
    \caption{\textbf{Effect of teacher trajectory curvature}. 
    (a) The student samples resemble the teacher ones for less curved trajectories. 
    (b) Straighter trajectories usually correspond to plainer teacher images.}
    \label{fig:curvature}
\end{figure} 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/no-ref.jpg}
    \caption{\textbf{Full-reference vs no-reference decision-making}. Usually, one can find a $k$-th percentile of the ImageReward scores providing the correlation with human votes similar to the full-reference comparisons but without observing the teacher samples.}
    %Usually, there is a percentile providing the same correlation as the full-reference estimate without seeing a teacher sample.}
    \label{fig:ref_no_ref}
\end{figure} 

To sum up, we conclude that the student largely diverges from the teacher on the samples that are challenging in different respects.
Interestingly, the superior student samples often occur in these cases.

% This behavior resembles deep ensembles~\cite{} where a bunch of independently trained models provide diverse predictions on the complex inputs and increase the overall performance.
% However, in our case, the distilled model initialized with the teacher weights and learnt to imitate the teacher still can produce sufficient diverse samples to significantly improve the teacher performance.
% We hypothesize that it is caused by the highly stochastic nature of the diffusion models and consistency distillation methods.

\subsection{Method}

In this section, we propose an adaptive collaborative approach consisting of three steps:
1) Generate a sample with the student model;
2) Decide if the sample needs further improvement;
3) If so, refine or regenerate the sample with the teacher model.

\textbf{Student generation step} produces an initial sample $\mathcal{X}^{\mathbf{S}}$ for a given context and noise.
This work considers consistency distillation~\cite{song2023consistency} as a primary distillation framework and uses multistep consistency sampling~\cite{song2023consistency} for generation. %\dmitry{what about ADD?}

\textbf{Adaptive step} leverages our finding that many student samples may exhibit superior quality.
Specifically, we seek an ``oracle'' that correctly detects superior student samples. 
For this role, we consider an individual sample quality estimator $\mathbf{E}$. 
In particular, we use the current state-of-the-art automated estimator, ImageReward (IR)~\cite{xu2023imagereward} that is learned to imitate human preferences for text-to-image generation.

Then, comparing the scores of the teacher and student samples, one can conclude which one is better.
However, in practice, we avoid expensive teacher inference to preserve the efficiency of our approach.
Therefore, a decision must be made having access only to the student sample $\mathcal{X}^{\mathbf{S}}$. 
To address this problem, we introduce a cut-off threshold $\tau$ which is a $k$-th percentile of the IR score tuned on a hold-out subset of student samples. 
The details on the threshold tuning are described in~\ref{app:method}.
During inference, the IR score is calculated only for $\mathcal{X}^{\mathbf{S}}$.
If it exceeds the threshold $\tau$, we accept the sample and avoid further teacher involvement. 
Interestingly, we observe that it is often possible to reproduce the accuracy of the full-reference estimation by varying $\tau$ (see \fig{ref_no_ref}). 
Also, note that IR calculation costs are negligible compared to a single diffusion step, see \ref{app:ir_inference_costs}.

\textbf{Improvement step} engages the teacher to improve the quality of the rejected student samples.
We consider two teacher involvement strategies: \textit{regeneration} and \textit{refinement}. 
The former simply applies the teacher model to produce a new sample from scratch for the same text prompt and noise.
The refinement is inspired by the recent work~\cite{podell2023sdxl}. 
Specifically, $\mathcal{X}^{\mathbf{S}}$ is first corrupted with a Gaussian noise controlled by the rollback value $\sigma \in [0, 1]$. 
Higher $\sigma$ leads to more pronounced changes. 
We vary $\sigma$ between $0.3$ and $0.75$ in our experiments.
Then, the teacher starts sampling from the corrupted sample following the original noise schedule and using an arbitrary solver, e.g., DPM-Solver~\cite{lu2022dpm}.
Note that refinement requires significantly fewer steps to produce the final sample than generation from scratch. 
Intuitively, the refinement strategy aims to fix the defects of the student sample.
At the same time, the regeneration strategy may be useful if $\mathcal{X}^{\mathbf{S}}$ is poorly aligned with the text prompt in general.
Our experiments below confirm this intuition.

==> sec/5_exps.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{images/image_synth_ours_teacher.jpg}
    \vspace{-2mm}
    \captionof{figure}{Visual examples produced with the proposed adaptive approach and the teacher model.} 
    \label{fig:ours_teacher_generation}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{images/all_metric.pdf}
    \vspace{-2mm}
    \captionof{figure}{\textbf{User preference results}. 
    (a) Comparison of NFE budgets when our approach performs on par with the top-performing teacher configuration.
    (b) Comparison to the teacher model with DPM-Solver under the same NFE budgets.
    (c) Comparison to the refinement strategy without the adaptive step under the same NFE budgets.
    (Top row) - LAION-Aesthetic text prompts. 
    (Bottom row) - COCO2014 text prompts.
    For our adaptive approach, we use the refinement strategy (R).
    } 
    \label{fig:users_study}
\end{figure*}

\section{Experiments}
We evaluate our approach for text-to-image synthesis, text-guided image editing and controllable generation. 
The results confirm that the proposed adaptive approach can outperform the baselines for various inference budgets. 

\subsection{Text-guided image synthesis} \label{subsec:image_synth}
In all experiments, we consider Stable Diffusion v1.5 as a teacher model and use the default classifier-free guidance scale 8. 
All generated images have $512{\times}512$ resolution.
As a student model, we implement consistency distillation (CD) for latent diffusion models and distill Stable Diffusion on the 80M subset of LAION2B~\cite{schuhmann2022laion}. 
The resulting model demonstrates decent performance for 5 steps of multistep consistency sampling with the guidance scale 8.
% \dmitry{We also provide the results for DreamshaperV7 and the corresponding distilled model in \app{}}
\\ \textbf{Metrics}. 
We first consider FID~\cite{heusel2017fid}, CLIP score~\cite{radford2021learning} and ImageReward~\cite{xu2023imagereward} as automatic metrics. 
ImageReward is selected due to a higher correlation with human preference compared to FID and CLIP scores.
ViT-g/14~\cite{zhai2022scaling} is used for CLIP score calculation. 
For evaluation, we use $5000$ text prompts from the COCO2014 validation set~\cite{lin2014microsoft}. 

Also, we evaluate user preferences using side-by-side comparisons conducted by professional assessors.
We select random $600$ text prompts from the COCO2014 validation set and $600$ prompts from LAION-Aesthetics\footnote{https://laion.ai/blog/laion-aesthetics/}.
More details are in~\ref{app:t2i}.
As a primary efficiency measure, we consider the number of function evaluations (NFE). 
% The COCO prompts lead to more realistic images, while the prompts from the second group - to more aesthetic ones. 
% In total, ${\sim}25,000$ comparisons were conducted.
\\ \textbf{Configuration}. 
For our adaptive approach, we consider both refinement (R) and regeneration (G) strategies using a second order multistep DPM solver~\cite{luu2022dpm}. 
We vary the number of sampling steps from $5$ to $45$ depending on the NFE budget. 
As a sample estimator $\mathbf{E}$, we consider ImageReward, except for the CLIP score evaluation. 
For each NFE budget, we tune the hyperparameters $\sigma$ and $\tau$ on the hold-out prompt set. 
The exact values are provided in~\ref{app:t2i}.
\\ \textbf{Baselines}. 
We consider the teacher performance as our main baseline and use DDIM~\cite{song2020denoising} for 50 NFE and a second order multistep DPM solver~\cite{luu2022dpm} for lower NFE regimes.  
In addition, we compare with the recent Restart Sampling~\cite{xu2023restart} and consider the refining strategy on top of the distilled model alone, without the adaptive step.
This choice is inspired by the recent results~\cite{podell2023sdxl} demonstrating the advantages of the refinement step itself. 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/automatic_t2i.pdf}
    \caption{{Comparison of the FID, CLIP and ImageReward scores for different NFEs on the 5K text prompts from COCO2014. 
    The proposed collaborative approach outperforms all the baselines.
    The adaptive pipeline with the teacher regeneration strategy (G) demonstrates higher textual alignment (CLIP score) while the refinement strategy (R) improves the image fidelity (FID).
    }}
    \label{fig:automatic_t2i}
\end{figure} 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/dynamic_acc.pdf}
    \caption{User preferences for the different accuracy levels of the sample estimator. 
    \textit{Current state} represents the results with the ImageReward estimator. 
    Other results demonstrate the potential gains if the estimator performance improves in the future.}
    \label{fig:perspectives}
\end{figure} 
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/ours_vs_teacher.jpg}
    \vspace{-5mm}
    \caption{Visual examples of our approach next to the top-performing teacher configuration. \textit{Top:} Text-guided image editing with SDEdit~\cite{meng2021sdedit}. \textit{Bottom:} Controllable image generation with Canny edges and semantic segmentation masks using ControlNet~\cite{zhang2023adding}.} 
    \label{fig:ours_teacher}
\end{figure*}
\\ \textbf{Results}. 
The quantitative and qualitative results are presented in Figures \ref{fig:users_study}, \ref{fig:automatic_t2i} and Figure \ref{fig:ours_teacher}, respectively. 
According to the automatic metrics, our approach outperforms all the baselines. 
Specifically, in terms of CLIP scores, the adaptive regeneration strategy demonstrates superior performance compared to the refining-based counterpart. 
On the other hand, the adaptive refining strategy is preferable in terms of FID scores. 
We assume that the refinement strategy essentially improves the image fidelity and does not significantly alter the textual alignment due to the relatively small rollback values.  
In terms of ImageReward, both adaptive strategies perform equally. 

In the human study, we consider two nominations: i) \textit{acceleration}, where our approach aims to reach the teacher performance at high NFE: 50 steps of DDIM or 25 steps of DPM; ii) \textit{quality improvement}, where the adaptive method is compared with the baselines under the same NFE budgets. 
The results for the acceleration nomination are presented in Figure \ref{fig:users_study}a.
The proposed method achieves the teacher performance with $5{\times}$ and up to $2.5{\times}$ fewer NFEs compared to DDIM$50$ and DPM$25$, respectively.
The results for the second nomination (Figure \ref{fig:users_study}b,c) confirm that our approach consistently surpasses alternatives under the same NFE.
In particular, our method improves the overall generative performance by up to $19 \%$ and $20 \%$ compared to the teacher and refining strategy without the adaptive step, respectively.
\\ \textbf{Effect of estimator accuracy}. 
The potential bottleneck of our approach is the poor correlation of existing text-to-image automated estimators with human preference.
% \dmitry{TODO: confirm this:}Previously, it was noted that their predictive accuracy is largely sensitive to the prompt set or assessor instructions~\cite{wu2023human}.
For example, ImageReward usually exhibits up to $65 \%$ correlation with the annotators. 
Here, we investigate the effect of the estimator accuracy on the performance of our scheme to reveal its potential if more accurate estimators are developed in future work. 
Figure \ref{fig:perspectives} presents our method performance for different estimator accuracy rates and demonstrates significant future gains even for the $75\%$ correlation.

% Finally, we investigate the influence of the text-to-image estimator on the performance of our adaptive pipeline.
% Previously, it was noted that the predictive accuracy of the text-to-image estimators largely depends on the prompt set, assessor instructions and other sensitive factors~\cite{hpsv2}.
% Currently, ImageReward demonstrates up to $65 \%$ correlation with human votes. 
% Thus, we would like to give an insight how the adaptive approach will perform if the estimator accuracy increases in the future work. 
% Figure \ref{fig:perspectives} presents our method performance for different estimator accuracy levels and demonstrates significant future gains of the propose pipeline.

\subsection{Text-guided image editing}
This section considers our approach for text-guided image editing using SDEdit \cite{meng2021sdedit}. 
We add noise to an image, alter the text prompt and denoise it using the student model first.
If the edited image does not exceed the threshold $\tau$, the teacher model is used for editing instead.
In the editing setting, we observe that the refinement strategy significantly reduces similarity with the reference image due to the additional noising step. 
Thus, we apply the regeneration strategy only.

\begin{table}[t!]
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{c c c c c } 
\bottomrule
{Method} & NFE & DINOv2 $\downarrow$ & ImageReward $\uparrow$\\
\hline 
\iffalse
CD  &$5$ & $0.674$ \small{$\pm \ .004$} &  $0.192$ \small{$\pm \ .037$} \\ 
DDIM  &$50$& $0.665$ \small{$\pm \ .007$}  &  $0.183$ \small{$\pm \ .024$} \\ 
DDIM &$25$ & $0.665$ \small{$\pm \ .002$} &  $0.183$ \small{$\pm \ .022$} \\ 
DPM &$25$ & $0.667$ \small{$\pm \ .005$} &  $0.179$ \small{$\pm \ .020$} \\ 
Refinement &$30$ & $0.710$ \small{$\pm \ .005$} & $0.383$ \small{$\pm \ .033$}  \\ 
\hline
Ours &$30$ & ${0.669}$ \small{$\pm \ .006$} &  ${0.281}$ \small{$\pm \ .008$}  \\
% Ours (IR + DINOv2) & $\mathbf{0.336}$ \small{$\pm \ .005$} &  $\mathbf{0.255}$ \small{$\pm \ .022$}  \\
\fi
CD         & 5  & \cellcolor[HTML]{f0ffcc}0.674 \small{$\pm \ $ .004} & \cellcolor[HTML]{ffcccd}0.192 \small{$\pm \ $.037} \\ 
DDIM       & 50 & \cellcolor[HTML]{ccffcc}0.665 \small{$\pm \ $ .007} & \cellcolor[HTML]{ffcccd}0.183 \small{$\pm \ $.024} \\ 
DDIM       & 25 & \cellcolor[HTML]{ccffcc}0.665 \small{$\pm \ $ .002} & \cellcolor[HTML]{ffcccd}0.183 \small{$\pm \ $.022} \\ 
DPM        & 25 & \cellcolor[HTML]{ccffcc}0.667 \small{$\pm \ $ .005} & \cellcolor[HTML]{ffcccd}0.179 \small{$\pm \ $.020} \\ 
Refinement & 30 & \cellcolor[HTML]{ffcccd}0.710 \small{$\pm \ $.005}  & \cellcolor[HTML]{ccffcc}0.383 \small{$\pm \ $.033}  \\ 
\hline
Ours       & 30 & \cellcolor[HTML]{ccffcc}0.669 \small{$\pm \ $.006} &  \cellcolor[HTML]{ffffcc}0.281 \small{$\pm \ $.008}  \\
\bottomrule
\end{tabular} 
}
\vspace{-2mm}
\caption{Comparison of SDEdit with different approaches in terms of reference preservation DINOv2 and editing quality (ImageReward) for the strength $0.6$.}
\label{table:editing_fixed}
\end{table}

As performance measures, we use ImageReward for editing quality and DINOv2~\cite{oquab2023dinov2} for reference preservation. 
For evaluation, $100$ text prompts from the COCO2014 dataset are manually prepared for the editing task. 
% Other settings are similar to Section \ref{subsec:image_synth}. 
\\ \textbf{Results}. 
Table \ref{table:editing_fixed} provides evaluation results for a SDEdit noising strength value $0.6$.
The proposed method demonstrates a higher ImageReward score compared to the baselines with similar reference preservation scores. 
% We observe that the refinement strategy significantly reduces similarity with the original image due to the additional noising step. 
% Thus, in these experiments, we consider the adaptive regeneration strategy only. 
% Secondly, we evaluate different estimators, including ImageReward and a combination of ImageReward and DINOv2. 
% We find that the second approach preserve the reference slightly better. 
In addition, we present the performance for different editing strength values in Figure \ref{fig:editing_curve}. 
Our approach demonstrates a better trade-off between reference preservation and editing quality. We provide qualitative results in Figure \ref{fig:ours_teacher}.
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/editing_curve.pdf}
    \caption{SDEdit performance for different strength values in terms of reference preservation (DINOv2) and editing quality (IR).} %trade-off curves for different strength values in $[0.3, 0.9]$.}
    \label{fig:editing_curve}
\end{figure} 

\subsection{Controllable image generation}
Finally, we consider text-to-image generation using Canny edges and semantic segmentation masks as an additional context and use ControlNet~\cite{zhang2023adding} for this task.
We use ControlNet pretrained on top of Stable Diffusion v1.5 and directly plug it into the distilled model.
Interestingly, the model pretrained for the teacher model fits the student model surprisingly well without any further adaptation.

For the teacher model, the default ControlNet sampling configuration is used: $20$ sampling steps of the UniPC~\cite{zhao2023unipc} solver. 
In our adaptive approach, we use the refinement strategy with $10$ steps of the same solver.
For performance evaluation, we conduct the human preference study for each task and provide more details in \ref{app:applications}.
\\ \textbf{Results.} 
According to the human study, our approach outperforms the teacher ($20$ NFE) by $10 \%$ ($10$ NFE) and $5 \%$ ($12$ NFE) for Canny edges and semantic segmentation masks, respectively.
The visual examples are in Figure \ref{fig:ours_teacher}. 


==> sec/5_exps_arxiv.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{images/image_synth_ours_teacher.jpg}
    \vspace{-2mm}
    \captionof{figure}{Qualitative comparison of our adaptive refinement approach to the SD1.5 teacher model.} 
    \label{fig:ours_teacher_generation}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{images/all_metric.pdf}
    \vspace{-2mm}
    \captionof{figure}{\textbf{User preference study (SD1.5)}. 
    (a) Comparison of our approach to the top-performing teacher configurations.
    (b) Comparison to the teacher model with DPM-Solver for the same average number of steps.
    (c) Comparison to the refinement strategy without the adaptive step for the same average number of steps.
    \textit{Top row:} LAION-Aesthetic text prompts. 
    \textit{Bottom row:} COCO2014 text prompts.
    For our adaptive approach, we use the refinement strategy (R).
    } 
    \label{fig:users_study}
\end{figure*}

\section{Experiments}
We evaluate our approach for text-to-image synthesis, text-guided image editing and controllable generation. 
The results confirm that the proposed adaptive approach can outperform the baselines for various inference budgets. 

\subsection{Text-guided image synthesis} \label{subsec:image_synth}
In most experiments, we use Stable Diffusion v1.5 (SD1.5) as a teacher model and set the classifier-free guidance scale to $8$.
% All generated images have $512{\times}512$ resolution.
To obtain a student model, we implement consistency distillation (CD) for latent diffusion models and distill SD1.5 on the 80M subset of LAION2B~\cite{schuhmann2022laion}. 
The resulting model demonstrates decent performance for $5$ steps of multistep consistency sampling with the guidance scale $8$.
\\ \textbf{Metrics}. 
We first consider FID~\cite{heusel2017fid}, CLIP score~\cite{radford2021learning} and ImageReward~\cite{xu2023imagereward} as automatic metrics. 
ImageReward is selected due to a higher correlation with human preferences compared to FID and CLIP scores.
OpenCLIP ViT-bigG~\cite{cherti2022reproducible} is used for CLIP score calculation. 
For evaluation, we use $5000$ text prompts from the COCO2014 validation set~\cite{lin2014microsoft}. 

Also, we evaluate user preferences using side-by-side comparisons conducted by professional assessors.
We select $600$ random text prompts from the COCO2014 validation set and $600$ from LAION-Aesthetics\footnote{https://laion.ai/blog/laion-aesthetics/}.
More details on the human evaluation pipeline are provided in~\ref{app:human_eval}. \vspace{4mm}
\\ \textbf{Configuration}. 
For our adaptive approach, we consider both refinement (R) and regeneration (G) strategies using a second order multistep DPM solver~\cite{luu2022dpm} and vary the number of sampling steps depending on the average inference budget. %from $5$ to $45$
As a sample estimator $\mathbf{E}$, we consider ImageReward, except for the CLIP score evaluation. 
For each inference budget, we tune the hyperparameters $\sigma$ and $\tau$ on the hold-out prompt set. 
The exact values are provided in~\ref{app:sd15_setup}.
\\ \textbf{Baselines}. 
We consider the teacher performance as our main baseline and use DDIM~\cite{song2020denoising} for 50 steps and a second order multistep DPM solver~\cite{luu2022dpm} for lower steps.  
In addition, we compare to the refining strategy on top of all student samples, without the adaptive step.
This baseline is inspired by the recent results~\cite{podell2023sdxl} demonstrating the advantages of the refinement stage itself.
Also, we provide the comparison with Restart Sampling~\cite{xu2023restart}.
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/automatic_t2i.pdf}
    \vspace{-6mm}
    \caption{{\textbf{Automated evaluation (SD1.5)}. Comparison of the FID, CLIP and ImageReward scores for different number of sampling steps on 5K text prompts from COCO2014. 
    The proposed collaborative approach outperforms all the baselines.
    The adaptive pipeline with the regeneration strategy (G) demonstrates higher textual alignment (CLIP score), while the refinement strategy (R) improves the image fidelity (FID).
    }}
    \label{fig:automatic_t2i}
\end{figure} 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/sdxl_res.pdf}
    \vspace{-6mm}
    \caption{
        \textbf{User preference study (SDXL).} 
        \textit{Left:} Comparison of the adaptive approach with CD-SDXL to the top-performing teacher setup. 
        \textit{Right:} Comparison of the adaptive approach with ADD-XL to ADD-XL for the same average number of steps.
    }
    \label{fig:sdxl_res}
\end{figure} 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/dynamic_acc.pdf}
    \vspace{-6mm}
    \caption{User preferences for different accuracy levels of the no-reference decision-making procedure.
    %the automated sample estimator. 
    \textit{Current state} represents the results using ImageReward. 
    The results for higher accuracy rates demonstrate the future gains if the oracle performance improves.}
    \label{fig:perspectives}
\end{figure} 
\\ \textbf{Results}. 
The quantitative and qualitative results are presented in Figures \ref{fig:users_study}, \ref{fig:automatic_t2i} and Figure \ref{fig:ours_teacher}, respectively. 
According to the automatic metrics, our approach outperforms all the baselines. 
Specifically, in terms of CLIP scores, the adaptive regeneration strategy demonstrates superior performance compared to the refining-based counterpart. 
On the other hand, the adaptive refining strategy is preferable in terms of FID scores. 
We assume that the refinement strategy essentially improves the image fidelity and does not significantly alter the textual alignment due to the relatively small rollback values.  
In terms of ImageReward, both adaptive strategies perform equally. 

In the human evaluation, we consider two nominations: i) \textit{acceleration}, where our approach aims to reach the performance of SD1.5 using $50$ DDIM steps or $25$ DPM steps; ii) \textit{quality improvement}, where the adaptive method is compared to the baselines for the same average number of steps. 
The results for the acceleration nomination are presented in Figure \ref{fig:users_study}a.
The proposed method achieves the teacher performance for $5{\times}$ and up to $2.5{\times}$ fewer steps compared to DDIM$50$ and DPM$25$, respectively.
The results for the second nomination (Figure \ref{fig:users_study}b,c) confirm that our approach consistently surpasses alternatives using the same number of steps on average.
In particular, the adaptive method improves the generative performance by up to $19\%$ and $20\%$ compared to the teacher and refining strategy without the adaptive step, respectively.
\\ \textbf{Effect of oracle accuracy}. 
The potential bottleneck of our approach is a poor correlation of existing text-to-image automated estimators with human preferences.
For example, ImageReward usually exhibits up to $65 \%$ agreement with annotators. 
Moreover, it remains unclear what oracle accuracy can be achieved with no-reference decision-making, even if the estimator provides the perfect agreement.

In \fig{perspectives}, we conduct a synthetic experiment examining the effect of the oracle accuracy on our scheme performance to reveal its future potential. 
% In \fig{perspectives}, we conduct a synthetic experiment examining the effect of the oracle accuracy on our scheme performance to reveal its future potential. 
%if more accurate estimators are developed in future work. 
We compare the adaptive refinement method ($10$ steps) to SD1.5 ($50$ steps) manually varying the oracle accuracy. 
We observe significant future gains even for the $75\%$ accuracy rate.
%Note that it remains unclear what level of accuracy can be achieved with no-reference decision-making even if the estimator provides the perfect agreement. %a perfect estimator is available.
\\ \textbf{SDXL results}. 
In addition to SD1.5 experiments, we evaluate our pipeline using the recent CD-SDXL~\cite{luo2023latent} and ADD-XL~\cite{sauer2023adversarial} which are both distilled from the SDXL-Base model~\cite{podell2023sdxl}. 
Our approach with CD-SDXL stands against the top-performing SDXL setting: $50$ steps of the DDIM sampler. 
For ADD-XL, we provide the comparison for $4$ steps where ADD-XL has demonstrated exceptionally strong generative performance in terms of human preference~\cite{sauer2023adversarial}.
In both settings, our approach uses the adaptive refinement strategy with the UniPC solver~\cite{zhao2023unipc}.
Note that both the SDXL-Base and SDXL-Refiner~\cite{podell2023sdxl} models can be used for refinement. 
In our experiments, we observe that the refiner suits slightly better for fixing minor defects while the teacher allows more pronounced changes. 
Thus, we use the refiner for low $\sigma$ values and the base model for the higher ones. %($\leq0.4$)
More setup details are provided in~\ref{app:sdxl_setup}.

The results are presented in \fig{sdxl_res}.
We observe that the adaptive approach using CD-SDXL achieves the quality of the SDXL model, being $5{\times}$ more efficient on average.
Moreover, the proposed scheme improves the performance of ADD-XL by $14\%$ in terms of human preference.

% \dmitry{todo: For refinement, we use the SDXL Refiner model. Note that the SDXL base model can also be used, but we observe that the refiner performs slightly better for low NFE settings.}
% For both cases, we compare our approach with the top-performing configurations: $50$ steps of the DDIM sampler using the SDXL model and $4$ steps of the ADD-XL. 
% For our approach, we consider the adaptive refinement strategy using UniPC solver~\cite{zhao2023unipc}.
% More details are in~\ref{app:t2i}.
%Note that the ADD-XL overcomes its teacher but suffers from mode collapse~\cite{goodfellow2020generative}. However, this is not the case for the CD~\cite{song2023consistency}, as we discuss in Section~\ref{sec:diversity}.
%we perform $4$ sampling steps with the student model and consider $12$ steps for the refinement strategy.
% As a result, the adaptive scheme with $70\%$ acceptance rate consumes $13$ NFE in total and we compare it with 
%Also, we compare our approach against ADD-XL using $4$ generation steps which has demonstrated higher human preferences than the teacher model~\cite{sauer2023adversarial}.
%In the adaptive setting, we consider $2$ steps of ADD-XL, $4$ refining steps and $50\%$ acceptance rate, resulting in $4$ NFE.
%In both evaluations, the guidance scale is $8$ for all models and SDXL Refiner~\cite{podell2023sdxl} is used for the refining strategy.


\subsection{Distribution diversity} \label{sec:diversity}
\begin{figure}[t!]
    \centering
    \vspace{-1mm}
    \includegraphics[width=0.99\linewidth]{images/diversity_final.pdf}
    \vspace{-3mm}
    \caption{Diversity human scores collected for different methods.}
    \label{fig:diversity_scores}
\end{figure}
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/app_corr_complexity.jpg}
    \vspace{-6mm}
    \caption{Image complexity of the CD-SD1.5 and SD1.5 samples in terms of ICNet~\cite{feng2023ic9600}. \textit{Left:} Box plot representing the complexity quantiles for both models. \textit{Right:} Distribution of individual complexity values. Each dot corresponds to a pair of samples generated for the same prompt and initial noise. The distilled model only slightly simplifies the teacher distribution.}
    \label{fig:app_student_compl}
    \vspace{-1mm}
\end{figure}

In the proposed teacher-student collaboration, the oracle aims to accept high-quality and well-aligned student samples but does not control the diversity of the resulting image distribution.
Therefore, if the student exhibits severe mode collapse or oversimplifies the teacher samples, the adaptive pipeline will likely inherit these issues to some extent.

In this section, we investigate this potential problem for several existing distilled text-to-image models. 
Specifically, we consider consistency distillation~\cite{luo2023latent} for SD1.5 and SDXL~\cite{podell2023sdxl} models and ADD-XL~\cite{sauer2023adversarial}. 
Note that ADD-XL is a GAN-based distillation method that generates exceptionally realistic samples but has evidence to provide poor image diversity for the given text prompt~\cite{sauer2023adversarial}.

We estimate the diversity of generated images by conducting a human study.
In more detail, given a text prompt and a pair of samples generated from different initial noise samples, assessors are instructed to evaluate the diversity of the following attributes: angle of view, background, main object and style.
For each model, the votes are collected for $600$ text prompts from COCO2014 and aggregated into the scores from 0 to 1, higher scores indicate more diverse images. 
The results are presented in Figure~\ref{fig:diversity_scores}.

CD-SDXL demonstrates significantly better diversity than ADD-XL but still produces less various images compared to the SDXL teacher.
CD-SD1.5 performs similarly to the SD1.5 teacher.
Also, both adaptive strategies increase the diversity of the SDXL student models, especially the regeneration one.
%Notably, the adaptive approach with CD-based students demonstrates comparable results to the corresponding teacher models. 
We also provide a few samples generated with different distilled models in~\ref{app:diversity}.

Then, we address whether the distilled models tend to oversimplify the teacher distribution.
In this experiment, we evaluate SD1.5 using DDIM for $50$ steps and the corresponding CD-SD1.5 using $5$ sampling steps.
In~\fig{app_student_compl}, we compare the complexity of the student and teacher samples in terms of the ICNet score~\cite{feng2023ic9600}.
We observe that CD-SD1.5 imperceptibly simplifies the teacher distribution. %and, as a result, does not bring noticeable negative distribution changes.

To sum up, in our experiments, the CD-based models provide the decent distribution diversity that can be further improved with the proposed adaptive approach. 

\subsection{Text-guided image editing}
\begin{figure*}[t!]
    \centering
    \vspace{-1mm}
    \includegraphics[width=0.99\linewidth]{images/ours_vs_teacher.jpg}
    \vspace{-2mm}
    \caption{Visual examples produced with our approach and the top-performing teacher (SD1.5) configuration. \textit{Top:} Text-guided image editing with SDEdit~\cite{meng2021sdedit}. \textit{Bottom:} Controllable image generation with Canny edges and semantic segmentation masks using ControlNet~\cite{zhang2023adding}.} 
    \label{fig:ours_teacher}
\end{figure*}
This section applies our approach for text-guided image editing using SDEdit~\cite{meng2021sdedit}. 
We add noise to an image, alter the text prompt and denoise it using the student model first.
If the edited image does not exceed the threshold $\tau$, the teacher model is used for editing instead.
In the editing setting, we observe that the refinement strategy significantly reduces similarity with the reference image due to the additional noising step. 
Thus, we apply the regeneration strategy only.

\begin{table}[t!]
\centering
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{c c c c c } 
\bottomrule
{Method} & Steps & DINOv2 $\downarrow$ & ImageReward $\uparrow$\\
\hline 
\iffalse
CD  &$5$ & $0.674$ \small{$\pm \ .004$} &  $0.192$ \small{$\pm \ .037$} \\ 
DDIM  &$50$& $0.665$ \small{$\pm \ .007$}  &  $0.183$ \small{$\pm \ .024$} \\ 
DDIM &$25$ & $0.665$ \small{$\pm \ .002$} &  $0.183$ \small{$\pm \ .022$} \\ 
DPM &$25$ & $0.667$ \small{$\pm \ .005$} &  $0.179$ \small{$\pm \ .020$} \\ 
Refinement &$30$ & $0.710$ \small{$\pm \ .005$} & $0.383$ \small{$\pm \ .033$}  \\ 
\hline
Ours &$30$ & ${0.669}$ \small{$\pm \ .006$} &  ${0.281}$ \small{$\pm \ .008$}  \\
% Ours (IR + DINOv2) & $\mathbf{0.336}$ \small{$\pm \ .005$} &  $\mathbf{0.255}$ \small{$\pm \ .022$}  \\
\fi
CD-SD1.5         & 5  & \cellcolor[HTML]{f0ffcc}0.674 \small{$\pm \ $ .004} & \cellcolor[HTML]{ffcccd}0.192 \small{$\pm \ $.037} \\ 
SD1.5, DDIM       & 50 & \cellcolor[HTML]{ccffcc}0.665 \small{$\pm \ $ .007} & \cellcolor[HTML]{ffcccd}0.183 \small{$\pm \ $.024} \\ 
SD1.5, DDIM       & 25 & \cellcolor[HTML]{ccffcc}0.665 \small{$\pm \ $ .002} & \cellcolor[HTML]{ffcccd}0.183 \small{$\pm \ $.022} \\ 
SD1.5, DPM        & 25 & \cellcolor[HTML]{ccffcc}0.667 \small{$\pm \ $ .005} & \cellcolor[HTML]{ffcccd}0.179 \small{$\pm \ $.020} \\ 
Refinement & 30 & \cellcolor[HTML]{ffcccd}0.710 \small{$\pm \ $.005}  & \cellcolor[HTML]{ccffcc}0.383 \small{$\pm \ $.033}  \\ 
\hline
Ours     & 30 & \cellcolor[HTML]{ccffcc}0.669 \small{$\pm \ $.006} &  \cellcolor[HTML]{ffffcc}0.281 \small{$\pm \ $.008}  \\
\bottomrule
\end{tabular} 
}
\caption{Comparison of SDEdit using different approaches in terms of reference preservation DINOv2 and editing quality (ImageReward) for the strength $0.6$.}
\label{tab:editing_fixed}
\end{table}

In these experiments, the SD1.5 and CD-SD1.5 models are considered.
As performance measures, we use ImageReward for editing quality and DINOv2~\cite{oquab2023dinov2} for reference preservation. 
For evaluation, $100$ text prompts from COCO2014 are manually prepared for the editing task. 
% Other settings are similar to Section \ref{subsec:image_synth}. 
\\ \textbf{Results}. 
\tab{editing_fixed} provides evaluation results for a SDEdit noising strength value $0.6$.
The proposed method demonstrates a higher ImageReward score compared to the baselines with similar reference preservation scores. 
% We observe that the refinement strategy significantly reduces similarity with the original image due to the additional noising step. 
% Thus, in these experiments, we consider the adaptive regeneration strategy only. 
% Secondly, we evaluate different estimators, including ImageReward and a combination of ImageReward and DINOv2. 
% We find that the second approach preserve the reference slightly better. 
In addition, we present the performance for different editing strength values in Figure \ref{fig:editing_curve}. 
Our approach demonstrates a better trade-off between reference preservation and editing quality. We provide qualitative results in Figure \ref{fig:ours_teacher}.
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/editing_curve.pdf}
    \vspace{-6mm}
    \caption{SDEdit performance for different strength values in terms of reference preservation (DINOv2) and editing quality (IR).} %trade-off curves for different strength values in $[0.3, 0.9]$.}
    \label{fig:editing_curve}
    \vspace{-1mm}
\end{figure} 

\subsection{Controllable image generation}
Finally, we consider text-to-image generation using Canny edges and semantic segmentation masks as an additional context and use ControlNet~\cite{zhang2023adding} for this task.
We use ControlNet pretrained on top of SD1.5 and directly plug it into the distilled model (CD-SD1.5).
Interestingly, the model pretrained for the teacher model fits the student model surprisingly well without any further adaptation.

For the teacher model, the default ControlNet sampling configuration is used: $20$ sampling steps of the UniPC~\cite{zhao2023unipc} solver. 
In our adaptive approach, we use the refinement strategy with $10$ steps of the same solver.
For performance evaluation, we conduct the human preference study for each task on $600$ examples and provide more details in \ref{app:applications}.
\\ \textbf{Results.} 
According to the human evaluation, our approach outperforms the teacher ($20$ steps) by $19 \%$ ($9$ steps) and $4 \%$ ($11$ steps) for Canny edges and semantic segmentation masks, respectively.
The visual examples are in Figure~\ref{fig:ours_teacher}. 



%\begin{table}[t!]
%\centering
%\resizebox{\linewidth}{!}{
%\begin{tabular}{c c | c c c | c} 
%\toprule
%Method & NFE & Viewpoint & Background & Main object  %& Avg\\
%\midrule
%CD-SDXL & $4$ & $0.547$ & $0.627$ & $0.753$ & %\cellcolor[HTML]{ffffcc}$0.642$\\
%Adaptive (R) & $9$ & $0.581$ & $0.666$ & $0.757$  & %\cellcolor[HTML]{f0ffcc}$0.668$\\
%Adaptive (G) & $29$ & $0.629$ & $0.604$ & $0.766$ & %$0.666$\\
%SDXL & $50$ & $0.670$ & $0.593$ & $0.762$ & %\cellcolor[HTML]{ccffcc}$0.675$ \\
%\midrule
%ADD-XL & $4$ & $0.314$ & $0.531$ & $0.637$ & %\cellcolor[HTML]{ffcccd}$0.494$\\
%Adaptive (R) & $4$ & $0.434$ & $0.476$ & $0.672$  & %$0.527$\\
%Adaptive (G) & $29$ &$0.471$ & $0.554$ & $0.665$ & %$0.563$\\
%SDXL & $50$ &$0.670$ & $0.593$ & $0.762$  & %\cellcolor[HTML]{ccffcc}$0.675$ \\
%\midrule
%CD-SD1.5 & $5$ &$0.620$ & $0.678$ & $0.918$ & %\cellcolor[HTML]{ccffcc}$0.738$\\
%Adaptive (R) & $12$ & TODO & TODO & TODO & TODO\\
%Adaptive (G) & $40$ & TODO & TODO & TODO  & TODO\\
%SD1.5 & $50$ & $0.658$ & $0.667$ & $0.917$ & %\cellcolor[HTML]{ccffcc}$0.747$\\
%\bottomrule
%\end{tabular}
%}
%\caption{.}
%\label{table:diversity}
%\end{table}


==> sec/X_suppl_arxiv.tex <==
\clearpage
\onecolumn

\setcounter{page}{1}

\newpage
\appendix
\maketitlesupplementary

% \section{Discussions}

% \textbf{Connection to LLM cascades.}
% The proposed adaptive approach resembles cascades of large language models (LLMs)~\cite{chen2023frugalgpt}, which have recently demonstrated its potential for cost-effective language modeling.
% Specifically, the pipeline usually combines cheap and expensive LLMs, e.g., GPT-J~\cite{gpt-j} and GPT-4~\cite{gpt4}. 
% The cheap model first generates the initial response to a user query; then, the answer scorer estimates if the response is fluent and accurate enough. 
% If not, the expensive model is queried to improve the response.

% This work shows that similar ideas can be naturally extended for text-conditional diffusion models as well.
% The key difference is that LLM cascades usually consider independently trained models while our approach uses the student and teacher models.
% We believe that this difference may be important in text-to-image generation.
% Therefore, it is interesting to investigate if other fast text-to-image methods, e.g., text-conditional GANs~\cite{kang2023gigagan, Sauer2023stylegant}, can be successfully applied instead of the distilled models.
% To the best of our knowledge, there are no publicly available text-conditional GANs or any other efficient text-to-image approaches to address this question, and hence we leave it for future work.

% Opposed to LLM cascades, which seek accurate responses within the particular downstream task, text-to-image generation aims to represent the original distribution in general.
% Thus, it gets interesting if any other fast text-to-image method, e.g., text-conditional GANs~\cite{kang2023gigagan, Sauer2023stylegant}, can be used instead of the distilled models.
% Thus, it gets interesting which text-to-image methods can be preferable as the first stage generators.
% We repute that the fast text-to-image alternatives need to demonstrate at least similar diversity to the expensive model to avoid negative distribution changes.
% Otherwise, the oracle will accept high quality and well-aligned images from the efficient model at the cost of the overall diversity.

% The proposed text-to-image pipeline runs the distilled model to produce initial samples.
% It gets interesting if any other fast text-to-image method can be used instead, e.g., text-conditional GANs~\cite{kang2023gigagan, Sauer2023stylegant}.
% Opposed to LLM cascades, which seek accurate responses within the particular downstream task, text-to-image generation aims to represent the original distribution.
% Therefore, we repute that fast text-to-image alternatives need to produce not only high fidelity images but also represent at least similar diversity to the expensive model.
% % Therefore, we repute that fast text-to-image alternatives need to produce not only high fidelity images but also represent at least similar diversity to the expensive model.
% Otherwise, the oracle likely accepts high quality and well-aligned images from the efficient model at the cost of the overall diversity.

% To the best of our knowledge, there are no publicly available text-conditional GANs or other efficient text-to-image approaches to investigate this question in detail.
% % Therefore, this question needs to be carefully addressed in future work.
% Nevertheless, we provide evidence that the current distilled models do not pose these issues.
% In \fig{app_student_compl} (Right), we plot the dependency between the student and teacher sample complexity in terms of~\cite{feng2023ic9600}.
% Each dot represents a pair of samples for the same prompt and initial noise.
% \fig{app_student_compl} (Left) presents the mean and standard deviation of the sample complexity.
% We observe that our student model does not tend to oversimplify the teacher images.


%the natural question is whether it is important to use the student model as an initial generator or
% To the best of our knowledge, the only publicly available highly efficient text-to-image generators are distilled diffusion models. 
% Opposed to LLMs seeking \textit{some} plausible response to the user query, 
% The fast model produces initial samples which serve as foundation 
% We repute that the primary condition to the fast alternative is to represent the similar image diversity to the slow model.  
% In text-to-image generation, it is important to produce diverse images for the given text prompt and do not oversimplify the samples in general. 
% For example, GANs often prefer image fidelity to diversity~\cite{dhariwal2021diffusion}. 
% Since the oracle needs to make a decision based on the initial sample only, it will likely accept high fidelity GAN images at the cost of overall diversity.

% Also, independent models have unaligned latent spaces and hence no-reference sample selection may be less effective 
% Intuitively, independent text-to-image models may cause undesired distribution changes.
% Since the oracle needs to make a decision based on the GAN sample only, it has no idea if the diffusion model would produce either higher quality or more expressive sample because the models are independent.
% In the result, the oracle will likely accept high fidelity GAN images at the cost of diversity.

% Unfortunately, to the best of our knowledge, there are no publicly available text-to-image GANs or other efficient approaches other than the distilled models to confirm this intuition.
% Therefore, this question needs to be carefully addressed in future work.

% Nevertheless, we provide the evidence that in the student-teacher collaborations, the student does not tend to oversimplify the teacher images, especially in the winning cases.
% In \fig{}, we plot the dependency between the student and teacher sample complexities under the same prompt and initial noise in terms of~\cite{feng2023ic9600}.
% Red dots correspond to the student wins, blue - teacher wins and gray - ties. 
% We observe that TODO

% \section{Societal Impact} \label{app:kal}

\section{CD-SD1.5 implementation details}
\label{app:student_details}
In this work, we develop consistency distillation (CD) for Stable Diffusion following the official implementation~\cite{song2023consistency}. 
For training, we prepare a subset of LAION2B~\cite{schuhmann2022laion}, which consists of $80$M image-text pairs. 
As a teacher sampler, we consider DDIM-solver using $50$ sampling steps and Variance-Preserving scheme~\cite{song2020score}. 
We use the teacher UNet architecture as a student model and initialize it with the teacher parameters. 
Classifier-free guidance is applied to the distilled model directly without merging it into the model as done in~\cite{meng2023distillation}. %the use of an additional distillation step
%We leave it for the future work. 
During training, we uniformly sample the guidance strength from $1$ to $8$. 
Thus, our model supports different guidance scales during sampling. 
We train the student for ${\sim}200$K iterations on $8$ A100 GPUs using the following setting: $512$ batch size; $0.95$ EMA rate; $1\text{e}{-}5$ fixed learning rate; L2 uniformly weighted distillation loss calculated in the latent space of the VAE encoder. 
During inference, the multistep stochastic sampler~\cite{song2023consistency} is used to generate images. 
In most of our experiments, we use $5$ sampling steps.

Note that we use our implementation of consistency distillation for SD because, when most experiments were conducted, there were no publicly available implementations. 


\begin{figure*}[t!]
    \centering
    \vspace{-2mm}
    \includegraphics[width=0.95\linewidth]{images/coco_compexity.jpg}
    \vspace{-3mm}
    \caption{SD1.5 samples of different complexity according to the ICNet model~\cite{feng2023ic9600}.}
    \label{fig:app_complexity}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/curv_coco_attn.jpg}
    \vspace{-6mm}
    \caption{\textit{Left}: Two examples of diffusion model trajectories with high and low curvatures. \textit{Right}: Trajectory deviations according to~\cite{chen2023geometric}.}
    \label{fig:app_curv}
\end{figure*}

\section{Analysis} \label{app:analysis}
\subsection{Calculation details}
\label{app:calc_details}
\textbf{Image complexity}. 
To calculate the image complexity, we use the recent ICNet model~\cite{feng2023ic9600}. 
This model is learned on a large-scale human annotated dataset. 
Each image corresponds to a complexity score ranging from 0 (the simplest) to 1 (the most complex). 
In Figure~\ref{fig:app_complexity}, we provide examples of Stable Diffusion samples with the lowest and highest image complexity. 
More complex images usually depict multiple entities, often including people, and intricate backgrounds.
\\ \textbf{Text influence}. 
We calculate the influence of a text prompt on student generation by using cross-attention between token embeddings and intermediate image representations. 
Following~\cite{tang2023daam}, we collect cross-attention maps for all diffusion steps and UNet~\cite{ronneberger2015u} layers. 
Then, the average attention score is calculated for each text token. 
Finally, the highest value among all tokens is returned.
\\ \textbf{Trajectory curvature} is estimated according to the recent work~\cite{chen2023geometric}. 
First, we calculate the trajectory deviations as L2 distance from the denoised prediction at a time step $t$ to the straight line passing
through the denoising trajectory endpoints. 
The trajectory curvature corresponds to the highest deviation over all time steps. 

In Figure~\ref{fig:app_curv} (Left), we visualize two denoising trajectories corresponding to high and low curvatures. 
We apply PCA~\cite{jolliffe2016principal} to reduce the dimensionality of the denoised predictions.
In addition, Figure~\ref{fig:app_curv} (Right) demonstrates trajectory deviations for different time steps. 
The highest deviations typically occur closer to the end of the denoising trajectory.

%\begin{figure*}
%    \centering
%    \includegraphics[width=\linewidth]{images/app_student_better.jpg}
%    \caption{Student outperforms its teacher according to the human evaluation.}
%    \label{fig:app_student_better2}
%\end{figure*}


\subsection{Other distilled text-to-image models}
\label{app:other_distill}
Here, we conduct a similar analysis as in Section \ref{main_analysis} for consistency distillation on Dreamshaper v$7$~\cite{luo2023latent} and architecture-based distillation\footnote{\url{https://huggingface.co/docs/diffusers/using-diffusers/distilled_sd}}.

In contrast to the few-step distillation approaches~\cite{meng2023distillation, song2023consistency, kim2023consistency, liu2022flow, luo2023latent}, the architecture-based distillation removes some UNet layers from the student model for more efficient inference and trains it to imitate the teacher using the same deterministic solver and number of sampling steps. 

In Figures~\ref{fig:app_dual_mode_dream_stable},~\ref{fig:app_dual_mode_arch}, we show that both methods can produce samples that significantly differ from the teacher ones for the same text prompt and initial noise. 
Then, Figures~\ref{fig:app_all_arch},~\ref{fig:app_all_lcm} confirm that other observations in Section~\ref{main_analysis} remain valid for the Dreamshaper and architecture-based students as well.

% \section{Method} 
% \label{app:method}
\begin{algorithm}[t!]
\DontPrintSemicolon
  \KwInput{$\mathbf{E}, \mathbf{S}, \mathbf{T} - $ estimator, student, teacher; \\ $\mathcal{I} - $ input; $\sigma, \tau - $ rollback value and cut-off threshold.}
  \vspace{1.5mm}
  $\hat{\mathcal{O}} = \mathbf{S}(\mathcal{I})$ \tcp*{Student prediction}
  \vspace{1.5mm}
  \If{$\mathbf{E}(\hat{\mathcal{O}}) < \tau$ } 
  {
    \vspace{1.5mm}
    \textit{Strategy 1}: \tcp*{Refinement}
       \ \ \ \ $\hat{\mathcal{O}}_{\sigma} = \sqrt{1 - \sigma} \cdot \hat{\mathcal{O}} + \sqrt{\sigma} \cdot \mathcal{Z}, \ \mathcal{Z} \sim \mathcal
       {N}(0,1)$ \\
       \ \ \ \ $\hat{\mathcal{O}} = \mathbf{T}(\mathcal{I}, \hat{\mathcal{O}}_{\sigma})$ \\
    \textit{Strategy 2}: \tcp*{Regeneration}
        \ \ \ \ $\hat{\mathcal{O}} = \mathbf{T}(\mathcal{I})$ 
  }
  {\Return{$\hat{\mathcal{O}}$}}
\caption{teacher-student adaptive collaboration}
\label{alg:method_alg}
\end{algorithm}

\newpage
\section{Cut-off threshold tuning}
\label{app:method}
%\subsection{Rollback value}
%Our approach uses two primary hyperparameters: $\tau$ (cut-off threshold) and $\sigma$ (rollback value). 
%The rollback value controls the corruption strength in the adaptive refinement stage and can be varied between $0$ and $1$. 
%$1$ corresponds to the complete noise without any %information about an original image and $0$ to an initial %image without noise.
%Both hyperparameters are tuned on a hold-out subset for a %specified metric, e.g., ImageReward. 

The cut-off threshold $\tau$ is used for the adaptive selection of student samples. 
It corresponds to the $k$-th percentile of the metric values calculated on validation student samples. 
$600$ and $300$ samples are generated for tuning on the COCO2014 and LAION-Aesthetics datasets, respectively. 
Note that the prompts used for tuning do not overlap with the test ones.
Then, we calculate an individual score, e.g., IR score, for each validation student sample and select the percentile based on an average inference budget or target metric value. 
For example, suppose we select the percentile given a $15$ step budget and intend to perform $5$ student steps and $20$ steps for the improvement strategy.
In this case, we have to select $\tau$ as a $50$-th percentile, which results in the final average number of steps: $5+0.5\cdot 20=15$.

During inference, we perform the adaptive selection as follows: if the score of the student sample exceeds $\tau$, 
we consider that this sample might be superior to the teacher one and keep it untouched. 
Otherwise, we perform an improvement step using the teacher model (refinement or regeneration).
The proposed pipeline is presented in Algorithm~\ref{alg:method_alg}.

\section{Experiments} 
\subsection{Human evaluation}
\label{app:human_eval}
To evaluate the text-to-image performance, we use the side-by-side comparison conducted by professional annotators. 
Before the evaluation, all annotators pass the training and undergo the preliminary testing. 
Their decisions are based on the three factors: textual alignment, image quality and aesthetics (listed in the priority order). 
Each side-by-side comparison is repeated three times by different annotators. 
The final result corresponds to the majority vote.

\subsection{Experimental setup (SD1.5)}
\label{app:sd15_setup}
% In this case, we use from $3$ to $5$ steps of the CD-SD1.5. 
% Then, we use a teacher model (SD 1.5) with DPM-Solver~\cite{luu2022dpm}, adaptively applying from $5$ to $45$ steps.
The exact hyperparameter values and number of steps used for the automated estimation (FID, CLIP score and ImageReward) of the adaptive refinement strategy in Table~\ref{app:tab_hypers}. 
The adaptive regeneration uses the same cut-off thresholds and number of steps, but the rollback value, $\sigma$, is equal to $1$.
The values used for human evaluation are presented in Table~\ref{app:tab_hypers_human}.

\subsection{Experimental setup (SDXL)}
\label{app:sdxl_setup}
We evaluate two distilled models: CD-SDXL~\cite{luo2023latent} and ADD-XL~\cite{sauer2023adversarial}. 
For the first evaluation, we use $4$ steps of the CD-SDXL and then apply $12$ adaptive refinement steps using the teacher model (SDXL-Base~\cite{podell2023sdxl}) with the UniPC solver~\cite{zhao2023unipc}. 
We compare our pipeline to the default teacher configuration: $50$ DDIM steps. 
For the second evaluation, we perform $2$ steps of the ADD-XL and $4$ steps of the SDXL-Refiner~\cite{podell2023sdxl} for the adaptive refinement strategy.
We compare to $4$ ADD-XL steps as this setting outperformed SDXL-Base in terms of image quality and textual alignment~\cite{podell2023sdxl}.
The exact hyperparameter values and number of steps used for human evaluation are in Table~\ref{app:tab_hypers_human_sdxl}.

We found that SDXL-Refiner performs slightly better than the base model for small refinement budgets (e.g., $4$). 
The refiner typically helps to improve fine-grained details, e.g., face attributes or background details.
However, it faces difficulties in providing global changes and sometimes brings artifacts for large rollback values, $\sigma$. 
Thus, we use the SDXL-Base teacher for more refinement steps (e.g., 12).


\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{} ll *{6}{c} @{}}
\toprule
Metric & $\sigma$
  & $k$
  & \multicolumn{3}{c}{Steps}\\
\cmidrule(l){4-6}
 & & &CD & Refinement & Adaptive\\
\midrule
ImageReward & $0.4$  & $60$ & $5$ & $5$  & $8$ \\
 & $0.55$  & $60$ & $5$ & $10$  & $11$ \\
 & $0.7$  & $60$ & $5$ & $15$  & $14$ \\
 & $0.7$  & $60$ & $5$ & $25$  & $20$ \\
 & $0.7$  & $60$ & $5$ & $35$  & $26$ \\
 & $0.7$  & $60$ & $5$ & $45$  & $32$ \\
\midrule
CLIP score & $0.5$  & $60$ & $5$ & $5$  & $8$ \\
 & $0.7$  & $60$ & $5$ & $10$  & $11$ \\
 & $0.75$  & $60$ & $5$ & $15$  & $14$ \\
 & $0.75$  & $60$ & $5$ & $25$  & $20$ \\
 & $0.75$  & $60$ & $5$ & $35$  & $26$ \\
 & $0.75$  & $60$ & $5$ & $45$  & $32$ \\
\midrule
FID & $0.75$  & $40$ & $3$ & $5$  & $5$ \\
 & $0.7$  & $70$ & $3$ & $15$  & $14$ \\
\bottomrule
\end{tabular} }
\vspace{-2mm}
\caption{Hyperparameter values used for the \textbf{automated evaluation (SD 1.5)}, Figure \ref{fig:automatic_t2i}.}
\label{app:tab_hypers}
\end{table}

\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{} ll *{6}{c} @{}}
\toprule
Metric & $\sigma$
  & $k$
  & \multicolumn{3}{c}{Steps}\\
\cmidrule(l){4-6}
 & & &CD &Refinement &Adaptive\\
\midrule
Human evaluation & $0.7$  & $50$ & $5$ & $10$  & $10$ \\
 & $0.7$  & $50$ & $5$ & $20$  & $15$ \\
 & $0.7$  & $50$ & $5$ & $40$  & $25$ \\
\bottomrule
\end{tabular} }
\vspace{-2mm}
\caption{Hyperparameter values used for the \textbf{user preference study (SD 1.5)}, Figure \ref{fig:users_study}.}
\label{app:tab_hypers_human}
\end{table}

\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{} ll *{6}{c} @{}}
\toprule
Metric & $\sigma$
  & $k$
  & \multicolumn{3}{c}{Steps}\\
\cmidrule(l){4-6}
 & & & ADD-XL &Refinement &Adaptive\\
\midrule
Human evaluation & $0.4$  & $50$ & $2$ & $4$  & $4$ \\
\toprule \toprule
&  & & CD-SDXL &Refinement &Adaptive\\
\midrule
Human evaluation & $0.85$  & $70$ & $4$ & $12$  & $13$ \\
\toprule
\end{tabular}  } 
\vspace{-2mm}
\caption{Hyperparameter values used for the \textbf{user preference study (SDXL)}, Figure \ref{fig:sdxl_res}.}
\label{app:tab_hypers_human_sdxl}
\end{table}

\subsection{Controllable generation}
\label{app:applications}
For both tasks, we use the adaptive refinement strategy and set the rollback value $\sigma$ to $0.5$.
We perform $5$ steps for the student generation and $10$ steps for the refinement with the UniPC solver.
The cut-off thresholds correspond to $70$ and $50$ ImageReward percentiles for the mask-guided and edge-guided generation, respectively.
We select random $600$ image-text pairs from the COCO2014 validation set for the edge-guided generation.
For the mask-guided generation, we use $600$ semantic segmentation masks from the ADE20K dataset~\cite{ade20k} and use the category names as the text prompts.  
To evaluate the performance, we conduct the human study similar to \ref{app:human_eval}.

\subsection{Distribution diversity} \label{app:diversity}
In Figure \ref{fig:diversity}, we illustrate the diversity of images generated with different distilled text-to-image models (ADD-XL, CD-SDXL and CD-SD1.5). 
Each column corresponds to a different initial noise (seed). 
We notice that ADD-XL exhibits the lowest diversity compared to the CD-based counterparts.

\subsection{ImageReward inference costs}
\label{app:ir_inference_costs}
We compare the absolute inference times of a single Stable Diffusion UNet step with classifier-free guidance against the ImageReward forward pass.
We measure the model performance in half precision on a single NVIDIA A100 GPU.
The batch size is $200$ to ensure $100\%$ GPU utility for both models.
The performance is averaged over $100$ independent runs.
ImageReward demonstrates $0.26$s while the single step of Stable Diffusion takes $3$s.
In the result, we consider the adaptive step costs negligible since ImageReward is more than $10{\times}$ faster than a single generation step of Stable Diffision.

\subsection{Additional visualizations}
In Figure \ref{fig:app_student_better1}, we present more examples where the student outperforms its teacher according to the human evaluation. 
Figures \ref{fig:app_editing_more}, \ref{fig:app_canny_more}, \ref{fig:app_segment_more} provide more qualitative comparisons of our approach for different tasks.


\begin{figure*}
    \centering
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.88\linewidth]{images/app_dual_mode.jpg}
         \caption{}
         \label{fig:app_dual_mode_stable}
     \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=0.88\linewidth]{images/app_dual_mode2.jpg}
         \caption{}
         \label{fig:app_dual_mode_dream}
     \end{subfigure}
     \caption{Visual examples of similar (Left) and dissimilar (Right) teacher and student samples for SD1.5 (a) and Dreamshaper v7 (b).}
     \label{fig:app_dual_mode_dream_stable}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=1.05\linewidth]{images/app_dual_mode3.jpg}
    \caption{Visual examples of similar (Left) and dissimilar (Right) teacher and student samples for the architecture-based distillation.}
    \label{fig:app_dual_mode_arch}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/app_all_arch.png}
    \caption{Analysis results for the architecture-based distillation.}
    \label{fig:app_all_arch}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/app_all_lcm.png}
    \caption{Analysis results for the consistency distillation on Dreamshaper v7.}
    \label{fig:app_all_lcm}
\end{figure*}

%\begin{figure*}
%    \centering
%    \includegraphics[width=\linewidth]{images/controllabel.pdf}
%    \caption{Student outperforms its teacher according to the human evaluation.}
%    \label{fig:app_control}
%\end{figure*}

% \section{Visualizations}
% In Figure \ref{fig:app_student_better1} we present  examples where the student outperforms its teacher according to the human evaluation. Moreover, 
% Figure \ref{fig:app_editing_more}, Figure \ref{fig:app_canny_more} and Figure \ref{fig:app_segment_more} demonstrates the qualitative results of our approach for different tasks.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/app_student_better_teacher.jpg}
    \caption{Additional examples where the student (CD-SD1.5) outperforms its teacher (SD1.5) according to the human evaluation.}
    \label{fig:app_student_better1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/ours_vs_teacher_editing.jpg}
    \caption{Additional image editing results produced with our approach.}
    \label{fig:app_editing_more}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/ours_vs_teacher_canny.jpg}
    \caption{Additional results on Canny edge guided image generation with our approach.}
    \label{fig:app_canny_more}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/ours_vs_teacher_segment.jpg}
    \caption{Additional results on segmentation mask guided image generation  with our approach.}
    \label{fig:app_segment_more}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.6\linewidth]{images/comp.jpg}
    \caption{Visual examples generated with various distilled text-to-image models for different seed values. CD-based students generate more diverse images than ADD-XL.}
    \label{fig:diversity}
\end{figure*}

\label{app:visualizations}

==> sec/discussion_and_limitations.tex <==
\section{Discussions and limitations}

The proposed approach essentially depends on the student model quality and the accuracy of the automated estimator. 
We believe that with a development of more advanced distillation techniques and accurate synthetic image assessment tools, the proposed pipeline may provide significantly stronger results.

In the future work, it is interesting to consider more sophisticated adaptive schemes, e.g., the collaboration between several students and their teacher, decide how many refinement steps are needed for a particular initial sample. 

Also, one can consider combining the expensive text-to-image diffusion models with other cheap text-conditional generative models, e.g., GANs.
We believe that the best initial cheap approximation is the one that preserves the diversity of the expensive model but has lower precision for some portion of samples. 
In this cases, the refinement stage can effectively improve the precision of low-quality samples but the overall diversity will be preserved.
In our opinion, the student models are the proper candidates for this role opposed to GANs that typically produce highly realistic images at the cost of diversity.
 
One could consider combining GANs with regeneration from scratch with diffusion models. However, it still poses two problems.
First, the latent spaces of different model types are not aligned and hence regeneration from scratch may produce entirely new sample which can be inferior to the initial one. 
Second, the automated assessment tools for individual samples do not estimate the diversity of generated samples. 
Therefore, if GANs produce high-quality samples of limited diversity, it is unlikely that the method decides to regenerate it with a more expensive model.
Nevertheless, the future work can address these problems and come up with novel adaptive pipelines with GANs and diffusion models.


==> sec/prev_method.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\linewidth]{images/student_better_teacher.pdf}
    \captionof{figure}{\textbf{Student outperforms its teacher}. We demonstrate this effect for the text-guided image synthesis (left) and image editing (right).} 
    \label{fig:student_better_teacher}
\end{figure*}

\section{Towards unified teacher-student framework}

Our goal is to find a diffusion-based approach which would demonstrate high efficiency and quality in applications (e.g., text-guided image synthesis, image editing, sketch-guided image generation). 
To that end, we first examine distilled models to identify their potential benefits for practice. 
Then, based on the findings, we propose an approach using adaptive collaboration of distilled and diffusion model.

To formalize the problem, let $\mathcal{I}$ be an input, e.g. prompt (for text-guided image synthesis), image and edited prompt (for image editing). The goal is to provide an output $\mathcal{O}$ having the highest user preference. Currently, a common way is to use diffusion-based approach, let $\mathbf{T}$ be a diffusion model (teacher) that produces $\hat{\mathcal{O}}_{\mathbf{T}} = \mathbf{T}(\mathcal{I}) \approx \mathcal{O}$. However, a serious drawback is the high computational cost associated with $\mathbf{T}$. To avoid this, there is a trend towards replacing the teacher with its distilled counterpart $\mathbf{S}$ (student). Unfortunately, high speed of $\mathbf{S}$ leads to a sacrifice in quality.

Our approach is orthogonal to the current trend. Specifically, instead of replacing $\mathbf{T}$ with $\mathbf{S}$, we are looking for an answer to the question: %\begin{tcolorbox}[colback=red!5!white,colframe=black!75!black]
 \textit{How to combine a teacher and student to achieve the highest performance in terms of quality and speed?}
%\end{tcolorbox} 
Our key observation is as follows:
\begin{tcolorbox}[colback=red!5!white,colframe=black!75!black]
A \textbf{student can surpass its teacher} despite the fact that the former learns to mimic the latter using less efforts. \end{tcolorbox} In other words, $\hat{\mathcal{O}}_{\mathbf{S}}$ demonstrates better performance than $\hat{\mathcal{O}}_{\mathbf{T}}$ for a substantial part of cases (up to $45 \%$). In Figure~\ref{fig:student_better_teacher} we provide some examples. We confirm our observation with user study (). More visualizations in \ref{app:visualizations}.

\subsection{Analysis} 
\begin{figure}[ht!]
    \centering
\includegraphics[width=1.0\linewidth]{images/dual_model_beh.png}
    \caption{(a) Dual-mode student behavior. (b) Differences between a student and a teacher leads to both quality improvement and degradation. (c) Human evaluation shows that if the student imitates the teacher, its win is insignificant and ties prevail. However, for the high distance, a student shows better results with a small number of ties.}
    \label{fig:dual_mode_beh}
\end{figure}
Here we aim to dive deeper into the found effect and reveal its nature.
\\ \textbf{Configuration}. For analysis we consider text-guided image synthesis problem. As a teacher we take Stable Diffusion v1.5 using 50 steps of DDIM. We focus on our realization of the Consistency Distillation. Moreover, we consider two others distillations in the supplement. To automatically measure the quality of outputs $\hat{\mathcal{O}}$ we use ImageReward (IR), which has shown a positive correlation with user preferences. To calculate the distance between $\hat{\mathcal{O}}_{\mathbf{T}}$ and $\hat{\mathcal{O}}_{\mathbf{S}}$ we take DreamSim (DS).  \\ 
\textbf{Dual-mode student behaviour}. Our second observation is the root cause of the effect we found: 
\begin{tcolorbox}[colback=red!5!white,colframe=black!75!black]
A \textbf{student works in two regimes}: {teacher-imitation} and {teacher-inimitable} (nado slovo drugoe) \end{tcolorbox}
We provide the visualizations of this finding in Figure \ref{fig:dual_mode_beh}a. In the teacher-imitation regime, a student produces outputs that are nearly identical to those of its teacher with only differences in fine-grained details. In this case, the portion of student wins is less significant (Figure \ref{fig:dual_mode_beh}c). On the other hand, there are student outputs that have significant changes in semantics and quality even for the same prompt. We claim that these changes can lead to both improvements and degradation compared to the teacher, which is confirmed in Figure \ref{fig:dual_mode_beh}b,c. Thus, in practice we aim to detect the positive changes in the student outputs and improve the negative ones using teacher. If we succeed, our approach will produce outputs better and faster than the teacher. Next, we consider some properties of the samples from these two groups.
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/complexity_distance_diverse.pdf}
    \caption{\textbf{Image complexity}. (a) The closer a student is to its teacher, the simpler the output is and vice versa. (b) Changes in quality (improvement and degradation) correspond to complex outputs.}
    \label{fig:image_complexity}
\end{figure} 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/prompts_analysis.pdf}
    \caption{\textbf{Prompts}. (a) The longer prompt usually leads to a higher teacher-student distance. However, it is not always true because of the prompt informativeness. (b) A student works as an independent model if the prompt influence weakens.}
    \label{fig:prompts}
\end{figure} 
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/curvature.pdf}
    \caption{\textbf{Trajectory curvature}. A student mimics its teacher for less curved trajectory. A more straight trajectory corresponds to simpler images.}
    \label{fig:curvature}
\end{figure} 
\\ \textbf{Image complexity}. Firstly, we investigate the correlation between the teacher-student distance and the complexity of teacher outputs. To compute the latter we use~\cite{feng2023ic9600}. The results are presented in Figure \ref{fig:image_complexity}. It can be noticed that a greater distance corresponds to a higher teacher complexity. In other words, a student mimic its teacher for simple concepts, like a close-up face. While for complex ones, a student generates in his own way, acting as a teacher independent model. Moreover, Figure \ref{fig:image_complexity}b confirms that significant changes in quality are observed for complex images. \\
\textbf{Prompts}. Secondly, we analyze the dual-mode student behaviour from a prompt perspective. Specifically, we explore the connection with prompt size and the impact of a prompt on a student output. To measure the latter, we aggregate the cross attention maps between an image and text during sampling by a student.

As it can be seen from Figure \ref{fig:prompts}a there is a positive correlation between the prompt size and teacher-student distance. However, the correlation accompanied by the high variance. We associate this with the possibility of long prompts being low in informativeness. That is, there is a non-zero probability that even for a long prompt, the teacher-student distance will be small, e.g. if a prompt is uninformative. 
Furthermore, Figure \ref{fig:prompts}c reveals that a student operates in the teacher-imitation regime if it relies heavily on a prompt.
\\ \textbf{Trajectory curvature}. Previously, it was shown that it is advantageous to straighten the trajectory of the
probability flows (\ref{background:reverse_ode}) before distillation~\cite{liu2022flow,liu2023instaflow}. The goal is to connect this findings with our observations. We calculate the curvature according~\cite{chen2023geometric}. 

Based on the results in Figure \ref{fig:curvature}, we can conclude the following: it is easier for a student to imitate a teacher if its outputs corresponds to a more straightened trajectory (low curvature). In addition, we show, for the first time, that the trajectory curvature correlates with the output complexity.

\subsection{Method}
In this section, we propose an adaptive collaborative approach consisting of three steps: 1) generate a sample with a student; 2) adaptively decide if a sample needs further improvements or not; 3) if so, improve a sample with a teacher model. 
\\ \textbf{Student generation step}. We use Consistency Distillation of Stable Diffusion with DDIM solver. 
Our implementation of CD supports the different guidance strengths. 
In practice, we use 5 steps of CD with the guidance strength equal to 8.
\\ \textbf{Adaptive step}. This part leverages our finding that a substantial portion of samples generated by a distilled model outperform the teacher ones.   
In practice, one needs an individual sample quality estimator, $\mathbf{E}$, producing reliable scores that correlate with human preference. Calculating this score for both teacher and student samples makes it possible to determine which one is better.
To that end, we consider the current state-of-the-art automated estimator, ImageReward~\cite{xu2023imagereward} that are learned to mimic the human preference. 

However, we face two challenges: 1) in practice, only the student output is known, while the teacher one is unavailable; 2) automatic quality estimators are far from perfect reproduction of human preferences, which limits the possible effectiveness of our approach. In particular, they exhibit up to $65 \%$ correlation with the annotators. 

To solve the first challenge, we introduce a cut-off threshold, $\tau$. If the quality of a student sample exceeds this threshold, we consider it to be a successful sample and vice versa. In practice, we consider the cut-off threshold as a $k$-th percentile of $\mathbf{E}$ tuned on a subset of samples.
We found that, usually, it is possible to perfectly reproduce the accuracy of full-reference estimation by varying $\tau$ (see Figure \ref{fig:ref_no_ref}). To address the second challenge, in \sect{todo} we consider the perspectives of our approach if the automated estimators potentially improves in future works. 
\\ \textbf{Improvement step}. This step is applied if the estimator recognize a sample of a student as unsuccessful, i.e. worse that a teacher. To improve the results we consider two strategies: refinement and re-generation using a teacher model. The former is inspired by the recent work~\cite{podell2023sdxl}. Specifically, we first generate the initial sample $\hat{\mathcal{O}}_{\mathbf{S}}$ using a distilled model. 
Then, we add a Gaussian noise controlled by the rollback value $\sigma$ according to (\ref{eq:forward_transition}). We vary this value between $0.4$ and $0.75$ in practice.
Finally, a teacher model starts the generation from the noised sample following an original noise schedule and using any solver, e.g., DPM-solver~\cite{lu2022dpm}.
In our experiments, we find that the first strategy better improves the image quality while the second one the textual alignment. The overall adaptive collaborative method is presented in \alg{method_alg}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{images/no-ref.pdf}
    \caption{\textbf{Full-reference vs no-reference}. Usually, there is a percentile providing the same correlation as the full-reference estimate without seeing a teacher sample.}
    \label{fig:ref_no_ref}
\end{figure} 

\begin{algorithm}[!ht]
\DontPrintSemicolon
  
  \KwInput{$\mathbf{E}, \mathbf{S}, \mathbf{T} - $ estimator, student, teacher; \\ $\mathcal{I} - $ input; $\sigma, \tau - $ rollback value and cut-off threshold.}
  \vspace{1.5mm}
  $\hat{\mathcal{O}} = \mathbf{S}(\mathcal{I})$ \tcp*{Student prediction}
  \vspace{1.5mm}
  \If{$\mathbf{E}(\hat{\mathcal{O}}) < \tau$}
  {
    \vspace{1.5mm}
    \textit{Strategy 1}: \tcp*{Refinement}
       \ \ \ \ $\hat{\mathcal{O}}_{\sigma} = (1 - \sigma) \cdot \hat{\mathcal{O}} + \sigma \cdot Z$ \tcp*{Noising}
       \ \ \ \ $\hat{\mathcal{O}} = \mathbf{T}(\mathcal{I}, \hat{\mathcal{O}}_{\sigma})$ \\
    \textit{Strategy 2}: \tcp*{Generation using teacher}
        \ \ \ \ $\hat{\mathcal{O}} = \mathbf{T}(\mathcal{I})$ 
  } 
  {\Return{$\hat{\mathcal{O}}$}}
\caption{teacher-student adaptive collaboration}
\label{alg:method_alg}
\end{algorithm}
